A Comparative User Study of Human Predictions in Algorithm-Supported Recidivism Risk Assessment

In this paper, we study the effects of using an algorithm-based risk assessment instrument to support the prediction of risk of criminalrecidivism. The instrument we use in our experiments is a machine learning version ofRiskEval(name changed for double-blindreview), which is the main risk assessment instrument used by the Justice Department ofCountry(omitted for double-blind review).The task is to predict whether a person who has been released from prison will commit a new crime, leading to re-incarceration,within the next two years. We measure, among other variables, the accuracy of human predictions with and without algorithmicsupport. This user study is done with (1)generalparticipants from diverse backgrounds recruited through a crowdsourcing platform,(2)targetedparticipants who are students and practitioners of data science, criminology, or social work and professionals who workwithRiskEval. Among other findings, we observe that algorithmic support systematically leads to more accurate predictions fromall participants, but that statistically significant gains are only seen in the performance of targeted participants with respect to thatof crowdsourced participants. We also run focus groups with participants of the targeted study to interpret the quantitative results,including people who useRiskEvalin a professional capacity. Among other comments, professional participants indicate that theywould not foresee using a fully-automated system in criminal risk assessment, but do consider it valuable for training, standardization,and to fine-tune or double-check their predictions on particularly difficult cases.

==> 02-related-work-OptB.tex <==
\section{Related work}
\label{sec:related-work}

\mynote[from=Manuel]{This is an optional distribution with 4 subsections, the "02-related-work" file is the original version from chato}
\subsection{Risk Assessment Instruments (RAI) for Criminal Recidivism}
\label{subsec:related-work-observational}

Law enforcement systems are increasingly using statistical algorithms to support individual release decisions by predicting the risk of offenders or arrestees to re-offend \cite{Goel2019,chiusi_automating_2020}.
%
Risk Assessment Instruments (RAIs) for criminal recidivism risk are in use in various countries including the U.S. \cite{desmarais2013risk}, the U.K. \cite{howard2012construction}, Canada \cite{kroner2007validity}, Austria \cite{rettenberger2010entwicklung}, Spain \cite{andres2018riscanvi} and Germany \cite{dahle2014development}, 
%
There are ethical and legal considerations regarding the use of statistics in decisions that affect human lives \cite{starr2014evidence}.
%
Some authors argue that fully automated decisions with algorithms that were trained on past human decisions may exhibit biases that were already present in data \cite{Angwin2016_machinebias,barocas2016big}. 
%
Others point out that, while this is true, there are potentially large welfare gains to the use of RAI that should also be considered \cite{kleinberg2018human}. 
%
%
According to the surveyed literature, decisions based on risks computed by RAIs in the jurisdictions where these instruments are used, are never made by an algorithm alone, but always involve a human in the decision making process.
%
The observed decisions, then, include partially elements that can be explained by the supporting RAI \cite{stevenson2021algorithmic}, and partially elements that can be traced back to the professionals (e.g. judges or case workers) that work with the RAI \cite{bao2021s}.
%
Because of this, algorithms aimed at supporting decision processes, especially in high-stakes contexts such as criminal justice, cannot be developed without taking into account the influences that institutional, behavioural and social aspects have on the decisions \cite{Selbst2019}. 
%
Therefore, some have studied the impact of the adoption of RAIs in criminal justice decision-making in real-world applications \cite{berk2017impact,stevenson2018assessing,stevenson2021algorithmic}.
%
A limitation of these studies, which are observational, is that the conditions of adoption as well as the design of the RAI cannot be controlled, making it difficult to disentangle the effect of various factors on the studied outcome.
%
%

\subsection{Controlled User Studies and Interaction Design of RAIs}
\label{subsec:related-work-experimental}

Algorithm-supported human decision making has also been studied in controlled experiments \cite{Dressel2018,Green2019,Green2019a,grgic2019human,Lin2020,fogliato2021impact}. 
%
Among these, an influential study by Dressel and Farid in 2018 \cite{Dressel2018}, showed how crowdsourcing workers recruited from Amazon Mechanical Turk (AMT) were able to outperform the predictions of COMPAS, a RAI that has been subject to significant scrutiny due to accusations of bias \cite{Angwin2016_machinebias}.
%
Follow-up studies criticized these findings arguing that in Dressel and Farid's study, participants were shown the ground truth of each case immediately after every prediction they make, which does not correspond to how these instruments are used in practice~\cite{Lin2020}.
%
Without this feedback, human predictions that were not supported by algorithms performed worse than the algorithm under analysis \cite{Lin2020}.
%
\inote{Manuel: I do not understand the next sentence, can you rephrase?}\inote{better?}
Similarly, \cite{Green2019a} also suggests that humans are unable to evaluate the performance of themselves or the risk assessment, and engage in "disparate interactions" reproducing biased predictions by the algorithm.
%do not recognize when algorithms err and underperform in the accuracy of their risk assessment, even with the help of algorithmic predictions.
%
%
\\
\subsection{Communicating Risk in RAIs}
\label{subsec:related-work-communication}

In general, there are many reasons why collaborative human-algorithm decisions deviates from pure algorithmic predictions. The way risk assessments are communicated and integrated in the decision process plays a crucial role in the quality of the predictions.
%
Sometimes, experts themselves may not know what is the best way of receiving risk assessments.
%
For instance, criminal forensics clinicians have a preference for (nonnumerical) categorical statements (such as low risk and high risk) over numerical risk levels  however, an experimental survey
%of 60 professionals reveals significant differences in the probabilities assigned by clinicians to certain categories, while numerical information alone led to a better performance of decision makers \cite{ZoeHilton2008}. 
showed that a RAI providing numerical information elicits better predictive accuracy than if categorical risk levels are used~\cite{ZoeHilton2008}. But numerical expressions are also controversial, some study participants perceive violence risk as higher when the risk is presented in a frequency format instead of a percentage format~\cite{Hilton2015}. Another question is whether numerical risks should be presented on an absolute or a relative scale. A study with different clinicians \cite{ZoeHilton2008} shows that participants hardly distinguish between absolute probability of violence and comparative risk.
%
The issue with categorical expressions is that professionals tend to disagree about the limits of the categories and how these categories represent different risk numerical estimations \cite{Hilton2015}.
%
With an intense debate about using the mere categorical level for professionals to reach a decision, \cite{Heilbrun1999} suggests that risk assessments may include other important detailed information on the nature of the crime, the factors of the RAI and other protective factors that may have preventive effects on future re-offense.
%
%Graphical representations, such as plots, are sometimes used to make numerical information easier to understand. Some authors included bar charts for comparing risk scores and graphical representations for categorical data, even if this requires stronger numeracy capacities, it appears as a potential improvement to ensure a common understanding on risk evaluations \cite{Hilton2017}. However, 
Complementary and graphical information can improve the understanding on risk evaluations \cite{Hilton2017}, but can also increase the overestimation of risk factors while ignoring other contextual information \cite{Batastini2019}. Nevertheless, the use of different visualization methods is mainly unexplored. 

\subsection{Human factors in algorithmic support systems}
\label{subsec:related-work-factors}
We also acknowledge that human factors such as biases, preferences and deviating objectives can also influence the effectiveness of algorithm-supported human decision making.
%

On the one hand, experienced decision makers may be more inclined to deviate from an algorithmic recommendation, relying more on their own cognitive processes \cite{Green2020}.
Moreover, probation officers prefer to rely in their own decision making, not just on a single numerical RAI prediction or the risk factors that are part of the RAI, but also let other, ``soft'' factors (e.g. empathy or motivations) influence their decisions. This additional information may even be used as a reason to override the RAI recommendation \cite{McCallum2017}. 

On the other hand, human decision-makers that are biased against certain groups produce biased decisions, independently of the design of the decision process \cite{jahanbakhsh2020experimental,Mallari2020}.
%

However, there can be other reasons to disagree with the algorithm recommendation, e.g., the human's objectives might be misaligned with the objective for which the algorithm is optimized \cite{Green2020a}, or the context which may create incentives for the human decision maker to deviate from the algorithm's recommendation, particularly if they perceive a misalignment of objectives \cite{stevenson2021algorithmic}.
%
Another reason could be algorithm aversion, i.e., human decision makers may discontinue the use of an algorithm after observing a mistake, even if the algorithm is on average more accurate than them \cite{dietvorst2015algorithm,burton2020systematic}.
%
That is, effective human-algorithm interaction also depends on user training with the tool and on the experience of the human decision maker with the algorithm, and on the specific professional domain in which the decision is made.

%%final remarks
Given the experience from previous works, we build our user interface to test and measure the performance of participants using different categorical risk levels and numerical expressions for risk, specifically absolute and relative risk scales.
%
We conduct the same re-offense prediction experiment with crowdsourced participants, as well as targeted participants.
%
This complements previous work by showing how targeted participants with a specific background in data science, or domain experts, perform differently than crowdsourced participants.
%
The additional focus group and interviews with professionals provide valuable insights into how RAIs are perceived and used in practice.

==> Riscanvi paper - experiment with humans/01-introduction.tex <==
\section{Introduction}
Since the 1970s the use of Risk Assessment Instruments (RAI) in high stakes contexts such as medicine or criminal justice, together with their risks and benefits, have been a subject of debate across various disciplines.
%
RAIs may increase the accuracy, robustness, and efficiency in decision making \cite{kleinberg2018human}; however, they can also lead to biased decisions and, consequently, to discriminatory outcomes \cite{Angwin2016_machinebias,skeem2016gender}. 
%
%

\begin{table}[t]
\hspace{-6mm}\begin{minipage}{0.48\linewidth}
    \centering\includegraphics[width=0.96\linewidth]{studies.pdf}
    
     \captionof{figure}{Sequence of studies and number of participants.}\label{fig:studies}
     \Description{The figure shows the three experimental studies (one targeted and two crowdsourced) and the different focus groups made during our study.}


\end{minipage}%
\hspace{2mm}%
\begin{minipage}{0.51\linewidth}
    \resizebox{1.02\linewidth}{!}{%
    \input{tab_demographics.tex}
    }\caption{Demographics by study group.}\label{tab:demographics}
%    
\end{minipage}
\vspace{-3pt}
 \end{table}

Understanding the performance of a RAI requires looking beyond the statistical properties of a predictive algorithm, and considering the quality and reliability of the decisions made \emph{by humans} using the RAI \cite{Green2021}.
%
This is because high-stakes decisions are rarely made by algorithms alone, and humans are almost invariably ``in-the-loop,'' i.e., involved to some extent in the decision making process \cite{Binns2021}.
%
Indeed, the General Data Protection Regulation (GDPR)\footnote{Available online: \url{https://eur-lex.europa.eu/legal-content/EN/TXT/?uri=CELEX\%3A32016R0679}. Accessed Jan 2022.} in Europe gives data subjects the right ``not to be subject to a decision based solely on automated processing'' (Article 22),
%
and the proposed Artificial Intelligence Act\footnote{Available online: \url{https://eur-lex.europa.eu/legal-content/EN/TXT/?uri=CELEX:52021PC0206}. Accessed Jan 2022.} published in April 2021, considers criminal risk assessment a ``high-risk'' application subject to stringent human oversight.
%

Our work involves a sequence of studies outlined in Figure~\ref{fig:studies} and described in the next sections. %sections~\ref{sec:approach}-\ref{sec:qualitative-study}.
%
We develop and test different user interfaces of a machine learning version of \RisCanvi, the main RAI used by \Catalonia's criminal justice system.\footnote{Name of instrument changed and name of country omitted for double-blind review.} 
%
%RisCanvi is based on factors that are empirically proven to affect the recidivism risk of individuals, such as their criminal history.
%
We ask participants to predict the re-incarceration risk based on the same factors used by \RisCanvi, such as criminal history, which empirically affect the recidivism risk of individuals.
%
Some participants are additionally shown the risk that the RAI predicts using the same factors.
%
Our primary goal is to assess how the interaction with the studied RAI affects human predictions, their accuracy, and their willingness to rely on a RAI for this task.
%

As most previous studies on this topic, we partially rely on crowdsourcing \cite{Dressel2018,Grgic-Hlaca2019,Green2020,fogliato2021impact}.
%, recruiting from the general population of workers available on a crowdsourcing platform.
%
%A major limitation of this approach is that these experiments
Controlled in-lab/survey experiments and crowdsourced experiments have the limitation that participants do not face the real world consequences that professional decisions have on the lives of inmates.
%
%A second limitation is that lay people 
In addition, untrained crowdworkers may exhibit different decision making behaviour than trained professionals. % working in the administration of justice.
%
The former limitation can only be addressed through studies that analyze the real-world adoption of a RAI through observational %and/or ethnographic 
methods \cite{berk2017impact,stevenson2018assessing,stevenson2021algorithmic}. However, these studies usually face the difficulty of isolating the effect of RAI adoption from other changes that co-occur in the study period.
%
%An example is the study by \citet{stevenson2021algorithmic}, who use historical data to retrospectively evaluate the impact of the adoption of a RAI in Virginia, USA, on variables such as the probability of incarceration and the length of a prison sentence.
%
%During the last decade, criminal systems around the globe experimented with algorithms with the intention to automate the process of evaluating the re-offense risk of defendants. %Although, in many instances, researchers found that such algorithms are biased, resulting in discriminatory outcomes. Moreover, in the scientific community it is known that the because of the contradictory nature of multiple moral and ethical concepts such as fairness and justice, can be operationalized all at once \cite{Green2020a}. As a result, we should consider that any future system will have a mixed approach, promoting collaboration between humans and algorithms at different levels and stages.\\
%
The latter can be addressed in an experimental setting by recruiting professional participants, as we do in this paper.
%
To the best of our knowledge, most studies focus on crowdsourced participants. This might be the first study that, in addition to a crowdsourced study, runs a targeted study. We recruited students and professionals of data science as well as domain experts (with a background in criminology and social work), including people who work within \Catalonia's criminal justice system and use \RisCanvi in a professional capacity. %The second goal of this study is to compare the performance of both groups.
%
Finally, we conducted a \emph{qualitative study} with small sub-groups of the targeted user study, particularly professionals %domain experts who use \RisCanvi in a professional capacity
within the Justice Department of \Catalonia, as well as data scientists. Our main contributions are:
\begin{itemize}
\item We confirm previous results that show how accuracy in decision making slightly improves with algorithmic support, how participants adjust their own predictions in the direction of the algorithmic predictions, and how different scales in risk communication yield different levels of accuracy.
\item We describe differences between targeted participants and crowdsourced workers. Despite identical experimental conditions and tasks, we find that the predictions differ between these groups and targeted participants outperform crowdsourced participants in terms of accuracy. 
%\item We acknowledge that domain experts and data scientists agree on giving relevance to same risk factors. Besides, domain experts self-reportedly focus more on dynamic risk-factors, and data scientists focused on static risk-factors.
\item We provide insights into how professionals use RAIs in real-world applications from our focus groups. Our interviewees would not foresee using a fully automated system in criminal risk-assessment, but they see benefits in using algorithmic support for training and standardization, and for fine-tuning and double-checking particularly difficult cases.
\end{itemize}

The remainder of this paper is structured as follows.
%
First, we give an overview of related work (\S\ref{sec:related-work}).
%
Next, we describe our approach, including the variables of our study (\S\ref{sec:approach}), as well as the materials and procedures we employ (\S\ref{sec:methods}).
%
We present the experiment setup for crowdsourced and targeted participants (\S\ref{sec:participants-and-exp-setup}), and the obtained results from both groups (\S\ref{sec:results}). Then we present the results from the focus groups (\S\ref{sec:qualitative-study}).
%
Finally, we discuss our findings  (\S\ref{sec:discussion}), as well as the limitations of this study and possible directions for future work (\S\ref{sec:limitations}).

==> Riscanvi paper - experiment with humans/02-related-work-OptB.tex <==
\section{Related work}
\label{sec:related-work}

\mynote[from=Manuel]{This is an optional distribution with 4 subsections, the "02-related-work" file is the original version from chato}
\subsection{Risk Assessment Instruments (RAI) for Criminal Recidivism}
\label{subsec:related-work-observational}

Law enforcement systems are increasingly using statistical algorithms to support individual release decisions by predicting the risk of offenders or arrestees to re-offend \cite{Goel2019,chiusi_automating_2020}.
%
Risk Assessment Instruments (RAIs) for criminal recidivism risk are in use in various countries including the U.S. \cite{desmarais2013risk}, the U.K. \cite{howard2012construction}, Canada \cite{kroner2007validity}, Austria \cite{rettenberger2010entwicklung}, Spain \cite{andres2018riscanvi} and Germany \cite{dahle2014development}, 
%
There are ethical and legal considerations regarding the use of statistics in decisions that affect human lives \cite{starr2014evidence}.
%
Some authors argue that fully automated decisions with algorithms that were trained on past human decisions may exhibit biases that were already present in data \cite{Angwin2016_machinebias,barocas2016big}. 
%
Others point out that, while this is true, there are potentially large welfare gains to the use of RAI that should also be considered \cite{kleinberg2018human}. 
%
%
According to the surveyed literature, decisions based on risks computed by RAIs in the jurisdictions where these instruments are used, are never made by an algorithm alone, but always involve a human in the decision making process.
%
The observed decisions, then, include partially elements that can be explained by the supporting RAI \cite{stevenson2021algorithmic}, and partially elements that can be traced back to the professionals (e.g. judges or case workers) that work with the RAI \cite{bao2021s}.
%
Because of this, algorithms aimed at supporting decision processes, especially in high-stakes contexts such as criminal justice, cannot be developed without taking into account the influences that institutional, behavioural and social aspects have on the decisions \cite{Selbst2019}. 
%
Therefore, some have studied the impact of the adoption of RAIs in criminal justice decision-making in real-world applications \cite{berk2017impact,stevenson2018assessing,stevenson2021algorithmic}.
%
A limitation of these studies, which are observational, is that the conditions of adoption as well as the design of the RAI cannot be controlled, making it difficult to disentangle the effect of various factors on the studied outcome.
%
%

\subsection{Controlled User Studies and Interaction Design of RAIs}
\label{subsec:related-work-experimental}

Algorithm-supported human decision making has also been studied in controlled experiments \cite{Dressel2018,Green2019,Green2019a,grgic2019human,Lin2020,fogliato2021impact}. 
%
Among these, an influential study by Dressel and Farid in 2018 \cite{Dressel2018}, showed how crowdsourcing workers recruited from Amazon Mechanical Turk (AMT) were able to outperform the predictions of COMPAS, a RAI that has been subject to significant scrutiny due to accusations of bias \cite{Angwin2016_machinebias}.
%
Follow-up studies criticized these findings arguing that in Dressel and Farid's study, participants were shown the ground truth of each case immediately after every prediction they make, which does not correspond to how these instruments are used in practice~\cite{Lin2020}.
%
Without this feedback, human predictions that were not supported by algorithms performed worse than the algorithm under analysis \cite{Lin2020}.
%
\inote{Manuel: I do not understand the next sentence, can you rephrase?}\inote{better?}
Similarly, \cite{Green2019a} also suggests that humans are unable to evaluate the performance of themselves or the risk assessment, and engage in "disparate interactions" reproducing biased predictions by the algorithm.
%do not recognize when algorithms err and underperform in the accuracy of their risk assessment, even with the help of algorithmic predictions.
%
%
\\
\subsection{Communicating Risk in RAIs}
\label{subsec:related-work-communication}

In general, there are many reasons why collaborative human-algorithm decisions deviates from pure algorithmic predictions. The way risk assessments are communicated and integrated in the decision process plays a crucial role in the quality of the predictions.
%
Sometimes, experts themselves may not know what is the best way of receiving risk assessments.
%
For instance, criminal forensics clinicians have a preference for (nonnumerical) categorical statements (such as low risk and high risk) over numerical risk levels  however, an experimental survey
%of 60 professionals reveals significant differences in the probabilities assigned by clinicians to certain categories, while numerical information alone led to a better performance of decision makers \cite{ZoeHilton2008}. 
showed that a RAI providing numerical information elicits better predictive accuracy than if categorical risk levels are used~\cite{ZoeHilton2008}. But numerical expressions are also controversial, some study participants perceive violence risk as higher when the risk is presented in a frequency format instead of a percentage format~\cite{Hilton2015}. Another question is whether numerical risks should be presented on an absolute or a relative scale. A study with different clinicians \cite{ZoeHilton2008} shows that participants hardly distinguish between absolute probability of violence and comparative risk.
%
The issue with categorical expressions is that professionals tend to disagree about the limits of the categories and how these categories represent different risk numerical estimations \cite{Hilton2015}.
%
With an intense debate about using the mere categorical level for professionals to reach a decision, \cite{Heilbrun1999} suggests that risk assessments may include other important detailed information on the nature of the crime, the factors of the RAI and other protective factors that may have preventive effects on future re-offense.
%
%Graphical representations, such as plots, are sometimes used to make numerical information easier to understand. Some authors included bar charts for comparing risk scores and graphical representations for categorical data, even if this requires stronger numeracy capacities, it appears as a potential improvement to ensure a common understanding on risk evaluations \cite{Hilton2017}. However, 
Complementary and graphical information can improve the understanding on risk evaluations \cite{Hilton2017}, but can also increase the overestimation of risk factors while ignoring other contextual information \cite{Batastini2019}. Nevertheless, the use of different visualization methods is mainly unexplored. 

\subsection{Human factors in algorithmic support systems}
\label{subsec:related-work-factors}
We also acknowledge that human factors such as biases, preferences and deviating objectives can also influence the effectiveness of algorithm-supported human decision making.
%

On the one hand, experienced decision makers may be more inclined to deviate from an algorithmic recommendation, relying more on their own cognitive processes \cite{Green2020}.
Moreover, probation officers prefer to rely in their own decision making, not just on a single numerical RAI prediction or the risk factors that are part of the RAI, but also let other, ``soft'' factors (e.g. empathy or motivations) influence their decisions. This additional information may even be used as a reason to override the RAI recommendation \cite{McCallum2017}. 

On the other hand, human decision-makers that are biased against certain groups produce biased decisions, independently of the design of the decision process \cite{jahanbakhsh2020experimental,Mallari2020}.
%

However, there can be other reasons to disagree with the algorithm recommendation, e.g., the human's objectives might be misaligned with the objective for which the algorithm is optimized \cite{Green2020a}, or the context which may create incentives for the human decision maker to deviate from the algorithm's recommendation, particularly if they perceive a misalignment of objectives \cite{stevenson2021algorithmic}.
%
Another reason could be algorithm aversion, i.e., human decision makers may discontinue the use of an algorithm after observing a mistake, even if the algorithm is on average more accurate than them \cite{dietvorst2015algorithm,burton2020systematic}.
%
That is, effective human-algorithm interaction also depends on user training with the tool and on the experience of the human decision maker with the algorithm, and on the specific professional domain in which the decision is made.

%%final remarks
Given the experience from previous works, we build our user interface to test and measure the performance of participants using different categorical risk levels and numerical expressions for risk, specifically absolute and relative risk scales.
%
We conduct the same re-offense prediction experiment with crowdsourced participants, as well as targeted participants.
%
This complements previous work by showing how targeted participants with a specific background in data science, or domain experts, perform differently than crowdsourced participants.
%
The additional focus group and interviews with professionals provide valuable insights into how RAIs are perceived and used in practice.

==> Riscanvi paper - experiment with humans/02-related-work.tex <==
\section{Related work}
\label{sec:related-work}

\subsection{Risk Assessment Instruments (RAI) for Criminal Recidivism}
\label{subsec:related-work-observational}

Law enforcement systems increasingly use statistical algorithms, e.g., methods that predict the risk of arrestees to re-offend, to support their decision making \cite{Goel2019,chiusi_automating_2020}. 
%
RAIs for criminal recidivism risk are in use in various countries including
Austria \cite{rettenberger2010entwicklung},
Canada \cite{kroner2007validity},
Germany \cite{dahle2014development}, 
Spain \cite{andres2018riscanvi},
the U.K. \cite{howard2012construction},
and
the U.S. \cite{desmarais2013risk}.
%
%There are ethical and legal considerations regarding the use of statistics in decisions that affect human lives \cite{starr2014evidence}.
%
There are ethical and legal aspects to consider, as algorithms may exhibit biases, which are sometimes inherited from the data on which they are trained \cite{barocas2016big}.  
%
However, some argue that RAIs bear the potential for considerable welfare gains \cite{kleinberg2018human}. 
%
The literature shows that decisions based on RAIs' scores are never made by an algorithm alone. Decisions in criminal justice are made by professionals (e.g., judges or case workers) \cite{bao2021s}, sometimes using RAIs  \cite{stevenson2021algorithmic}.
%
%
%Because of this, a
Consequently, algorithms aimed at supporting decision processes, especially in high-risk contexts such as criminal justice, cannot be developed without taking into account the influences that institutional, behavioural, and social aspects have on the decisions \cite{Selbst2019}. 
%
Furthermore, human factors such as biases, preferences and deviating objectives can also influence the effectiveness of algorithm-supported decision making~\cite{jahanbakhsh2020experimental,Mallari2020}.
%
%Human decision makers that are biased against certain groups may produce biased decisions, which can also influence the effectiveness of algorithm-supported decision making~\cite{jahanbakhsh2020experimental,Mallari2020}. %\inote{From F: Although [44] is a great study, I am not sure how it connects to real-world decision-making given that their experiments involved crowdworkers (who are making predictions). Same issue with the citation of [27] in the next line.}
%

%
% THE FOLLOWING IS ABOUT
% WHY DECISION MAKERS DEPART FROM ALGO RECOMMENDATIONS
%
Experienced decision makers may be more inclined to deviate from an algorithmic recommendation, relying more on their own cognitive processes \cite{Green2020}.
%
Moreover, trained professionals, such as probation officers, may prefer to rely on their own decision and not just on a single numerical RAI prediction. %or the risk factors that are part of the RAI, but also let other, ``soft'' factors (e.g. empathy or motivations) influence their decisions. 
Any additional information that they consider may be used as a reason to deviate from what a RAI might recommend for a case \cite{McCallum2017}. 
%
%However, t
There are other reasons why humans disagree with an algorithmic recommendation.
%
For instance, the human's objectives might be misaligned with the objective for which the algorithm is optimized \cite{Green2020a}, or the context may create incentives for the human decision maker not to follow the algorithm's recommendation \cite{stevenson2021algorithmic}. %, particularly if they perceive a misalignment of objectives 
%
%Reference \cite{Green2019a} also suggests that 
Sometimes humans are unable to evaluate the performance of themselves or the risk assessment, and engage in "disparate interactions" reproducing biased predictions by the algorithm~\cite{Green2019a}.
%do not recognize when algorithms err and underperform in the accuracy of their risk assessment, even with the help of algorithmic predictions.
%\inote{From F: In both works by Green and Chen ([25, 26]), the vignettes and survey designs were identical. I have been wondering for a while whether their result around disparate interactions of [25, 26] are simply artifacts of the survey design that they employ. In our work, for example, we have found no evidence of such interactions (section B.3 in our paper). Do you have some hints on why this might be the case?}
%
%
Another reason could be algorithm aversion, e.g., human decision makers may discontinue the use of an algorithm after observing a mistake, even if the algorithm is on average more accurate than them \cite{dietvorst2015algorithm,burton2020systematic}.
%
% THE FOLLOWING IS ABOUT
% WHY CROWDSOURCING WORKERS FOLLOW ALGO RECOMMENDATIONS
%
In contrast, controlled user studies in criminal risk assessment indicate that crowdsourced participants tend to exhibit \emph{automation bias}, i.e., a tendency to over-rely on the algorithm's prediction \cite{Dressel2018, Bansak2019}.
%

%
% IN SUMMARY
%
Effective human-algorithm interaction depends on users' training with the tool, on the experience of the human decision maker with the algorithm, and on the specific professional domain in which the decision is made.
%
Therefore, some researchers have studied the impact of the adoption of RAIs in criminal justice decision-making in real-world applications \cite{berk2017impact,stevenson2018assessing,stevenson2021algorithmic}.
%
These observational studies yield valuable insights, but the conditions of adoption as well as the design of the RAI cannot be controlled, making it difficult to isolate the effect of the RAI on the studied outcome.
%

\subsection{Controlled User Studies and Interaction Design of RAIs}
\label{subsec:related-work-experimental}

Algorithm-supported human decision making has also been studied in controlled experiments \cite{Dressel2018,Green2019,Green2019a,grgic2019human,Lin2020,fogliato2021impact}. 
%
Among these, an influential study by Dressel and Farid in 2018 \cite{Dressel2018}, showed how crowdsourced users recruited from Amazon Mechanical Turk (AMT) were able to outperform the predictions of COMPAS, a RAI that has been subject to significant scrutiny since the seminal work of Angwin et al.~\cite{Angwin2016_machinebias}.
%
Follow-up studies criticized Dressel and Farid's study, noting that participants were shown the ground truth of each case (i.e., whether or not the person actually recidivated) immediately after every prediction they make, which does not correspond to how these instruments are used in practice. %~\cite{Lin2020}.
%
Without this feedback, human predictions that were not supported by algorithms performed worse than the algorithm under analysis \cite{Lin2020}.
%

The way risk assessments are communicated and integrated in the decision process plays a crucial role in the quality of the predictions.
%
For instance, criminal forensics clinicians have a preference for (non-numerical) categorical statements (such as ``low risk'' and ``high risk'') over numerical risk levels. However, an experimental survey
%of 60 professionals reveals significant differences in the probabilities assigned by clinicians to certain categories, while numerical information alone led to a better performance of decision makers \cite{ZoeHilton2008}. 
showed that a RAI providing numerical information elicits better predictive accuracy than if categorical risk levels are used~\cite{ZoeHilton2008}. One issue with categorical expressions is that professionals tend to disagree about the limits of the categories and how these categories represent different numerical risk estimations \cite{Hilton2015}.
%
%\inote{finish talking about the drawbacks of categorical only before talking about the drawbacks of numerical --ChaTo}
%
However, numerical expressions introduce other challenges. For instance, participants in a study perceived violence risk as higher when the risk was presented in a frequency format instead of a percentage format~\cite{Hilton2015}.
%
Another question is whether numerical risks should be presented on an absolute or a relative scale.
%
A study with clinicians showed that participants hardly distinguish between absolute probability of violence and comparative risk \cite{ZoeHilton2008}.
%
%
%
%With an intense debate about using the mere risk level for professionals to reach a decision,
Furthermore, besides showing only risk levels, risk assessments could include additional information about the nature of the crime, the factors of the RAI and other factors that may have preventive effects on future re-offense~\cite{Heilbrun1999}.
%Graphical representations, such as plots, are sometimes used to make numerical information easier to understand. Some authors included bar charts for comparing risk scores and graphical representations for categorical data, even if this requires stronger numeracy capacities, it appears as a potential improvement to ensure a common understanding on risk evaluations \cite{Hilton2017}. However, 
Complementary and graphical information can improve the understanding of risk evaluations \cite{Hilton2017}.
%
However, it can also increase the overestimation of risk factors while ignoring other contextual information \cite{Batastini2019}. Nevertheless, the use of different visualization methods is mainly unexplored. 

%%final remarks
Given the experience from previous work, we build our user interface to test and measure the performance of participants using different categorical risk levels and numerical expressions for risk, specifically absolute and relative risk scales.
%
We conduct a recidivism prediction experiment with crowdsourced participants, but also complement it with targeted participants.
%
One of the main novelties of our study resides in assessing how targeted participants, including domain experts and data scientists, perform differently than crowdsourced participants.
%
Additionally, focus groups and interviews with professionals provide valuable insights into how RAIs are perceived and used in practice.

==> Riscanvi paper - experiment with humans/03-approach.tex <==
\vspace{-2mm}
\section{Approach and research questions}
\label{sec:approach}

%The research we describe in \S\ref{sec:approach}-\S\ref{sec:results} uses 
This paper takes an experimental approach.
%
Participants in our experiments are asked to determine the probability that an inmate will be re-arrested, based on a list of criminologically relevant characteristics of the case.
%
We focus on three main outcome variables (\S\ref{subsec:outcomes}): the accuracy of predictions, the changes that participants make to their predictions when given the chance to revise them after seeing the RAI's recommendation, and their willingness to rely on similar RAIs.
%
The main independent variables (\S\ref{subsec:conditions}) are the background of the participants, and the type of risk scale used.
% 
Our research questions (\S\ref{subsec:research-questions}) are about the interaction of these variables.

\subsection{Outcome variables}
\label{subsec:outcomes}

\subsubsection{Predictive accuracy}

The performance of predictive tools including RAIs is often evaluated in terms of the extent to which they lead to correct predictions. 
%
Due to the inherent class imbalance in this domain, as most people do not recidivate, most studies (e.g., experimental \cite{Dressel2018,Harris2015,Green2019}) do not use the metric \emph{accuracy}, which is the probability of issuing a correct prediction.
%
Instead, it is more common to measure the area under the receiver operating characteristic (\textbf{AUC-ROC} or simply \textbf{AUC}).
%
%The AUC can be interpreted as the probability that, given a positive item and a negative item (e.g., a person who recidivates and a person who does not), the RAI outputs a higher risk for the positive item than for the negative item.
The AUC can be interpreted as the probability that a randomly drawn recidivist obtains a higher score than a randomly drawn non-recidivist.
%
%This allows us to state our first research question.

\subsubsection{Prediction alignment with the RAI}
% I was willing to call this "reliance on this RAI" but thought I needed to be more precise -- ChaTo
%
In this work, we observe users' reliance on the algorithmic support system indirectly by looking at changes in their predictions after observing an algorithmic prediction.
%
We assume that if users change their initial predictions to align them with those of a RAI, they are implicitly signaling more reliance on that RAI than if they would have stuck to their initial prediction.
%
In general, the extent to which people are willing to trust and rely on a computer system is related to people's engagement and confidence in it \cite{VanMaanen2007,Chancey2017,Lee2004},
%
and in the case of predictive algorithms, to their perceived and actual accuracy~\cite{Yin2019}.
%
Different types of information disclosure can elicit different levels of trust and reliance~\cite{Du2019}. 
%
Performing joint decisions, i.e., being the human in the loop~\cite{De-Arteaga2020}, can increase willingness to rely on a system~\cite{Zhang2020}. 

\subsubsection{Preferred level of automation}\label{sec:level_automation}

The experience of interacting with an algorithm-based RAI may also affect the acceptability of similar algorithms in the future. Algorithm-based RAIs may operate in ways that differ by their \emph{level of automation}~\cite{Cummings2004}.
%
At the lowest level of automation, the human makes all decisions completely disregarding the RAI;
%
at the highest level of automation, the RAI makes all decisions without human intervention;
%
intermediate levels represent various types of automated interventions.
%
% OMIT THE NEXT LINE IF THIS EXPLAINED ELSEWHERE
%The specific description of these levels can be found in Appendix \ref{ann:automationlevel}. 
% 
In general, the level of automation chosen by a user should be proportionate to the performance of the automated system.
%
%\emph{Automation bias} happens when users rely on a system in a manner that is disproportionately large in comparison with the system's observed performance.
%
Both \emph{algorithm aversion} \cite{burton2020systematic} or under-reliance, as well as \emph{automation bias} \cite{Mosier1998} or over-reliance, negatively affect the predictive accuracy of users. %, who do not recognize and correct errors made by the automated system.
%
%The user study on criminal recidivism by Dressel and Farid \cite{Dressel2018} and its follow-up commentary \cite{Bansak2019} point out that crowdsourcing participants tend to exhibit automation bias.

\subsection{Participant groups and conditions}
\label{subsec:conditions}

In this section we describe the main independent variables that we tested in the experiments.

\subsubsection{Participant's educational and professional background} 
%
Most user studies on recidivism risk prediction rely on crowdsourced participants from online platforms.
%
The background of participants may change the way they interact with a RAI.
%
Data scientists and statisticians have training on statistics, probability, and predictive instruments.
%
Domain experts with a background in psychology, criminology, or who work within the prison system, have a deeper knowledge of factors driving criminal recidivism. 
%
Additionally, domain experts who use RAIs receive training on their usage, and they often have a fair amount of training in applied statistics.%, particularly in the case of psychologists and criminologists.
%
%

Naturally, in real-world applications case worker decisions are far more consequential than the consequences faced by crowdworkers in their lab-like decision scenarios.
%
Similar to previous work \cite{Green2019a, Cheng2019, Yu2020, Dressel2018}, we add an incentive (in the form of a bonus payment) for correct predictions in the crowdsourced studies. However, this is to encourage appropriate effort, not to simulate a high-stakes scenario.
%

We consider three participant groups: (1) crowdsourced workers from unspecified backgrounds, (2) students and practitioners of data science, and (3) students of criminology and people with expertise in the prison system. Recruitment procedures are described in \S\ref{subsec:participant-recruitment}.

\subsubsection{Risk scales}

The literature on risk communication suggests that both numerical and categorical information are useful for different purposes \cite{ZoeHilton2008, Jung2013, McCallum2017, Storey2015}.
%
Categories alone can be misleading when similar cases are assigned to different categories despite only small differences in their risk \cite{Jung2013}. 
%
In our research, we initially used only a categorical scale,\footnote{We group probabilities using a five-level, empirically-grounded recommendation developed by the US Department of Justice and the US National Reentry Resource Center~\cite{Hanson2017}.} but then switched to  scales that combine both categorical and numerical values; further, we test two different types of numerical scales.
%
The first scale is based on the probability of recidivism, which we denote ``absolute scale'' as it expresses a probability in absolute terms.
%
The second scale we use is based on quantiles of the risk distribution in the data, and we call it the ``relative scale'' since it is relative to the risk levels of other cases in the data. 
%
We also use five categories, for easier comparison with the absolute scale.
%
\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{scales.pdf}
\captionof{figure}{Risk scales used in our experiments (left: absolute scale, right: relative scale).}
\Description{Shows two different images with the interface where participants can set their prediction. Each image corresponds to different treatment group.\inote{mistake in computatiobal}}
\label{fig:scales}
\vspace{-3pt}
\end{figure}
%
%
Both scales are depicted in Figure~\ref{fig:scales}. Other elements in that figure are discussed in the following sections.
    
\subsubsection{Additional variables}
\label{subsubsec:additional-variables}

Many additional variables could have been included but we were mindful of survey length and wanted to minimize survey drop-out. 
%
We included three additional variables: numeracy, decision-making style, and current emotional state.
%
Numeracy is the ability to understand and manage numerical expressions.
%
The decision confidence and the type of information that professionals rely on when using RAIs depends on their numerical proficiency \cite{Scurich2015}.
%
Ideally, professionals working with RAIs should have a fairly high level of numerical literacy, as interpreting RAIs requires the understanding of probabilities, which is not common knowledge. 
%
Other factors that have been shown to affect people's decision making behaviour
are their decision-making style and current emotional state~\cite{Beale2008, Lee2012}.
%

\subsection{Research questions}
\label{subsec:research-questions}

Based on the variables we have presented, we pose the following research questions:

\begin{itemize}
\item[\textbf{RQ1}] \textbf{Under which conditions do participants using a RAI to predict recidivism achieve the highest predictive accuracy?}
\item[\textbf{RQ2}] \textbf{To what extent do participants rely on the RAI to predict recidivism?}
\end{itemize}


==> Riscanvi paper - experiment with humans/04-methods.tex <==
\section{Materials and methods}
\label{sec:methods}

In this section, we describe the materials (\S\ref{subsec:materials}) for our user study which consist of a risk prediction instrument based on \RisCanvi (\ref{subsubsec:riscanvi}) and a selection of cases used for assessment (\ref{subsubsec:cases}).
%
Next, we present a description of the procedure followed by participants (\ref{subsec:procedure}), and the way in which they were recruited (\ref{subsec:participant-recruitment}).

\subsection{Materials}\label{subsec:materials}

\subsubsection{\RisCanvi}\label{subsubsec:riscanvi}

This is one of several risk assessment tools used by the Justice Department of \Catalonia since %2009 and used across
2010 \refomitted{andres2018riscanvi}. 
%
This tool is applied multiple times during an inmate's time in prison; in most cases, once every six months.

%This is one of several violence risk assessment tools used by the Justice Department of \Catalonia since 2009 and used across all prisons in the system since 2010 \refomitted{andres2018riscanvi}. 
%
%This protocol is applied multiple times during an inmate's time in prison; the official recommendation is every six months or at the discretion of the case manager.
%
\RisCanvi consists of 43 items that are completed by professionals based on an inmate's record and suitable interviews. 
%This is not a questionnaire.
%
Then, a team of professionals (with some overlaps with the various interviewers) makes a decision based on the values of the items and the output of \RisCanvi's algorithm.
%
\RisCanvi's algorithm predicts the risks of four different outcomes: %\inote{From F: This is a subtle point, but participants are probably asked to predict re-arrest (which is what the RAI is predicting) and not re-offense. I have worked for a while on this issue so I care very much about the distinction: re-arrest is generally a very poor proxy of re-offense, e.g., see here https://arxiv.org/abs/2105.04953}
committing further violent offenses (violent recidivism),
violence in the prison facilities to other inmates or prison staff,
self-injury,
and breaking of prison permits. 
%A fifth risk score was introduced more recently for general recidivism \cite{singh2018handbook}.
%
We focus on \emph{violent recidivism}, which is computed based on 23 of the 43 risk factors, including
criminal/penitentiary record,
biographical factors, 
family/social factors,
clinical factors,
and attitude/personality factors. 
%
%These items can also be divided into static factors (such as criminal history of family and age of starting violent activity) and dynamic  factors (such as member of socially vulnerable groups and pro-criminal or antisocial  attitudes).

The original \RisCanvi uses integer coefficients determined by a group of experts; instead, we use a predictor of violent recidivism created using logistic regression that has a better AUC (0.76) than the original \RisCanvi (0.72) % The 0.72 is from karimi2021enhancing Table 1
and is more accurate than models created using other ML methods such as random forests or neural networks~\refomitted{karimi2021enhancing}.
%
This is done to reduce any effects of potential shortcomings of \RisCanvi originating from using hand-picked integer coefficients, instead using a state-of-the-art predictor based on the same items.

% executive report for riscanvi http://cejfe.gencat.cat/web/.content/home/recerca/cataleg/crono/2015/taxa_reincidencia_2014/tasa_reincidencia_2014_informe_ejecutivo.pdf

\subsubsection{Cases} \label{subsubsec:cases}

In this study, we use a dataset of cases used in previous work ~\refomitted{karimi2021enhancing}. It consists of the \RisCanvi protocol items for the inmates released between 2010 and 2013, and for which recidivism was evaluated by the Department of Justice of \Catalonia.
%
Upon recommendation of our Ethics Review Board, we do not show participants the data of any individual inmate, but instead created semi-synthetic cases using a cross-over of cases having similar features and similar risk levels %and run a preliminary study to evaluate predictive accuracy on humans %, which are a cross-over of similar cases having the same risk level 
%\mynote[from=Marzieh]{please check my note regarding "predictive accuracy" in Appendix~\ref{ann:casesel}.}
(for details, see Supplementary Material~\ref{ann:casesel}). 
%

%We created a large pool of such cases and performed a preliminary study in which we measured the predictive accuracy of humans and the algorithm on these cases (Appendix~\ref{ann:casesel}).
% 
We selected 14 cases which contain a mixture of recidivists and non-recidivists, combining cases in which the majority of humans make correct predictions and cases in which they tend to err, and cases in which the algorithm makes a correct prediction and cases in which it errs.
%
In our first crowdsourcing experiment (referred to as R1 in the following) we observed that these cases were not representative of the performance of the algorithm on the overall dataset. Hence, for the second crowdsourcing experiment (R2 in the following) we exchanged 2 cases to bring the AUC from 0.61 to 0.75 which is closer to the AUC of the algorithm on the original data (0.76).
%
Out of the 14 cases, 3 were used as examples during the ``training'' phase of the experiments, while participants were asked to predict recidivism for the remaining 11 cases.
%
All participants evaluate the same 11 cases, but in randomized order.

\subsection{Procedure} \label{subsec:procedure}

The study obtained the approval of our university's Ethics Review Board in December, 2020. 
%
All user studies were conducted between December, 2020 and July, 2021, and done remotely due to the pandemic caused by the SARS-COVID-19 virus. 
%
The survey is designed to be completed in less than 30 minutes and used an interface hosted in our university's server created using standard web technologies (Python and Flask).
%
The survey is structured as follows:

\subsubsection{Landing page and consent form}
%
The recruitment (\S\ref{subsec:participant-recruitment}) leads potential participants from different groups to different landing pages, which record which group the participant belongs to.
%
There, participants learn about the research and we ask for their explicit consent for participating.

\subsubsection{Demographics and additional variables}
Consenting participants are asked three \emph{optional} demographic questions: age (range), gender, and educational level.
%
Then, three sets of questions are asked to capture the following additional variables (described in \S\ref{subsubsec:additional-variables}):
%understand participant's personality (Results from these tests can be found in the Appendix \ref{ann:additionalresults}): 

\noindent- \emph{Numeracy}: We use a test by Lipkus \cite{Lipkus2001}, which has been used in previous work~\cite{Hilton2017}.
%
It consists of three questions about probabilities, proportions, and percentages, such as 
%
``If a fair dice is rolled 1,000 times, how many times it will come even (2, 4, or 6)?'' (Answer: 500).
%
We measure ``numeracy'' as the number of correct answers (0 to 3).

\noindent- \emph{Decision making style}: The General Decision Making  Style (GDMS)~\cite{Scott1995} is a well known survey that    identifies five types of individual decision making style: rational, intuitive, dependent, avoidant, and         spontaneous.  

\noindent- \emph{Current emotional state}: We used a Visual Analogue Scale (VAS) to account for 7 attitudes (happiness, sadness, anger, surprise, anxiety, tranquility, and vigor). This survey has been used in previous work~\cite{Portela2017}.
%to evaluate the individual disposition towards autonomous interfaces~\cite{Portela2017}.

\subsubsection{Past experience and attitudes towards RAIs}

Participants are asked about their knowledge about and experience with RAIs, as well as what they consider as the three most determining features to predict recidivism, out of the ones used by \RisCanvi.
%
The final question of this part is about the level of automation they would prefer for determining the risk of recidivism (see Supplementary Material \ref{ann:automationlevel}). 

\subsubsection{Training}

The training part consists of the risk assessment of three cases (two non-recidivists and one recidivist).
%
The purpose of this part is to prepare participants for the actual evaluations and to calibrate their assessment to a ground truth reference. 
%
Therefore, unlike the actual risk assessments of the evaluation tasks, participants are shown the ground truth (recidivism or no-recidivism) after each one. 

\subsubsection{Evaluation tasks}

The evaluation tasks are the core part of the study and ask participants to predict the probability of violent recidivism for eleven cases.
%
Participants see a list of 23 items that are used by \RisCanvi to predict violent recidivism (see Supplementary Material \ref{ann:surveytemplate} for an illustrated reference), and they are asked to select a number, which can be a recidivism probability or a risk level, depending on the condition (see Figure \ref{fig:scales}).
%
Additionally, they are asked to select from the list of items the three items that they considered most important in their evaluation, and to indicate their confidence with their prediction on a 5-points scale.
%

Participants in the control group are shown just one screen per case to enter their prediction, while participants in a treatment group are shown a second screen for each case, displaying the algorithm's prediction. % in comparison to their own prediction, on the same reference scale.
%
This second screen also shows participants their initial prediction for comparison, and allows them to optionally change it.
%
In both screens, participants indicate the confidence in their prediction before continuing. 

\subsubsection{Closing survey}

The experiment ends with a final questionnaire and an evaluation of the entire process.
%
This questionnaire repeats some of the questions made in the beginning, such as the preferred level of automation, the emotional state, and the three features they consider most important in predicting recidivism. 
%
Additionally, participants can leave a comment or feedback about the study. 

\subsection{Participant recruitment}\label{subsec:participant-recruitment}

A summary of the participants' demographics is shown in Table \ref{tab:demographics}.
%
The crowdsourced study consisted of two rounds (\textbf{R1} and \textbf{R2}) for which we recruited participants via Prolific.\footnote{Prolific is a crowdsourcing platform specialized in supporting scientific research. It is available at: https://www.prolific.co/} We selected residents of \Catalonia, %Actually: Spain
between 18 to 75 years old, and with more than 75\% of successful completion of other studies in the platform.
%
Participants were payed a platform-standard rate of 7.5 GBP\footnote{Prolific is a UK-based company that uses British pounds as main currency. We follow their advice for average payment per hour.} per hour for participating in the survey.
%
They took an average of 20$-$25 minutes to complete the survey. Additionally, we offered a bonus payment of 1 GBP to those who achieved an AUC greater than 0.7. 
%
This is common practice and incentivizes conscientious completion of the survey (see, e.g., \cite{Green2019a, Cheng2019, Yu2020, Dressel2018}).

For the targeted studies, participants were recruited through students' mailing lists from two universities in \Catalonia, as well as social media groups of professionals of data science in countries having the same official language as \Catalonia. % ARGENTINA AND CHILE
Additionally, we invited professionals from the Justice Department of \Catalonia to participate; the invitation to participate was done by their Department of Research and Training. %ADD THIS: and the Centre for Legal Studies and Specialised Training (CEJFE) from the Catalonia regional government. 
The number of participants in previous crowdsourced user studies is usually a few hundred: 103 in \cite{Grgic-Hlaca2019}, 202 in \cite{Cheng2019}, 400 in \cite{Lin2020}, 462 in \cite{Dressel2018} and 600 in \cite{Green2019a}. 
 %
In line with the previous studies, we had 449 participants in total (393 crowdsouced and 54 targeted). 


==> Riscanvi paper - experiment with humans/05-ALT-setup.tex <==
\section{Participants and experimental setup}
\label{sec:participants-and-exp-setup}

\subsection{Crowdsourced: First Round (R1)}
\label{sec:crowdsourced-study}
In the \textbf{first round} (R1) we compared two experimental groups. The  \textbf{treatment} group was  shown the machine prediction and the \textbf{control} group was not.
%
In treatment group \textbf{G1} machine predictions are shown only as \emph{categorical} information, while in \textbf{G2} machine predictions are shown as \emph{categorical and numerical} information.
% 
In this round, 247 participants completed the evaluation: 48 in the control group, 100 in treatment group G1, and 99 in treatment group G2. 
%\todo[from=Marzieh]{In Figure~\ref{fig:studies}, number of cases in R1 is 274 but here you wrote 247. Which one is the correct one? Please modify accordingly.}
%
Additionally, 74 participants were excluded, either because they did not complete the survey or did not evaluate all of the eleven cases, or finished the experiment either too fast (less than five minutes) or too slowly (more than one hour).
%

As described in \S\ref{subsubsec:cases}, we used in R1 a set of cases for which the AUC of the machine predictions was 0.61. 
%
To bring this more in line with the observed AUC in the entire dataset (0.76), we exchanged two cases for the second round (R2), and the AUC measured on the new set of cases became 0.75.

\subsection{Crowdsourced: Second Round (R2)}
\label{sec:crowdsourced-study-second-round}
\smallskip\noindent In the \textbf{second round} (R2) we compared two experimental groups, where the \textbf{treatment} group was shown the machine prediction and the \textbf{control} group was not.
%
In treatment group \textbf{G1} machine predictions are shown on an \emph{absolute scale} as categorical and numerical information, while in \textbf{G2} machine predictions are shown on a \emph{relative scale} as categorical and numerical information.

In this round, 146 participants completed the evaluation: 17 in the control group, 66 in treatment group G1, and 63 in treatment group G2. 
%
%Like in R1, 137 (GC:12, G1:61, G2:64) participants did not finish the experiment or were excluded.
Additionally, 137 participants were excluded for the same reasons as in R1.
%\mynote[from=Marzieh]{The total included participants are 474 (420+54). So is the original total number of participants about 685? (from which 74 and 137 participants were excluded from R1 and R2 respectively). > 658 = 247+146+29+25+74+137}

\subsection{Targeted Study}
\label{sec:targeted-study}

The targeted study seeks to establish the effect (if any) of the participant's background when interacting with the RAI.
%
We used the same experimental setup and treatment groups from crowdsourcing (R2).
%
Due to the limited number of participants, we considered as a baseline the control group of R2.

We considered both students and professionals with a background either in data science, or in a field relevant to the prison system and the application of \RisCanvi, such as psychology, criminology, or social work.
%
For data science, we recruited 14 students at the undergraduate and graduate level, and 11 professionals.
%
For a domain-specific background, we recruited 4 students at the graduate level (Master in Criminology students), and 25 professionals. 
%
A summary of all experimental groups is shown in Table~\ref{tab:experimentalgroups}.

==> Riscanvi paper - experiment with humans/06-ALT-results.tex <==
\section{Results}
\label{sec:results}
\subsection{Outcome variables}
\subsubsection{Predictive accuracy}

\begin{figure}[!tbp]
  \centering
  \begin{minipage}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{auc_group.pdf}
  \caption{Average AUC with 95\% confidence interval by group. See Table \ref{tab:results1} in Supplementary Material~\ref{ann:accuracy-per-subgroup} for details.}
  \Description{Shows a bar plot comparing each of the experimental groups, comparing their AUC-ROC before presenting the algorithm prediction and after.}
  \label{fig:auc_group}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{distance_to_algo.pdf}
  \caption{Average difference between human and algorithm prediction by case order, absolute scale.}\label{fig:learning}
  \Description{Shows a line graph where the initial prediciton made by humans is compared with the afterwards, lines are also split between crowdsourced and targeted studies.}
  \end{minipage}
\end{figure}
%\inote{From F: * section 5.2.4: These are pretty large differences in the AUC, so they might be meaningful despite not being statistically significant (you may simply lack power). How was the statistical significance of differences in the AUCs tested? I see a Welch t-test mentioned in Figure 5, but this is not valid because the AUCs of the participants are not normally distributed (given that you only have 11 examples, the distribution is discrete). Do you use a permutation test?
%* I am slightly concerned about the lack of power to detect meaningful changes when reading the results in sections 5 and 6}
Figure~\ref{fig:auc_group} shows the average AUC and corresponding confidence intervals\footnote{Confidence intervals in Figure~\ref{fig:auc_group} are computed under normal assumption but we test statistical significance of the differences using a permutation t-test (see Table \ref{tab:ttests})} for each experimental group. This data can also be found in Supplementary Material~\ref{ann:accuracy-per-subgroup}.
%
%In general, we observe no differences in the \emph{initial} predictions across control and treatment groups, which have AUC between 0.58 and 0.61.
For R1 we observe no difference in the \emph{initial} predictions across control and treatment groups, which have AUC between 0.58 and 0.61. However, for R2 we find a significant difference (p<0.1) with a higher AUC for the control group (0.65) than for the \emph{initial} prediction of treatment group G1 (0.58) with the absolute scale. %A reason for this could be that this treatment group operates in anticipation of algorithmic support and the option to revise the initial prediction. }

Despite the small number of participants in the targeted group, we observe important differences compared to the previous groups. The predictive accuracy of the initial prediction is higher (+0.02 to +0.09 AUC points) than any crowdsourced group. For the targeted group G1 (absolute scale) this difference is significant at %$p<0.09$
$p<0.1$ against R2's G2 and even at $p<0.05$ against the initial predictions of the other crowdsourced groups (see Supplementary Material~\ref{ann:accuracy-per-subgroup}).
%
Participants from a data science background and domain experts have similar initial AUCs. 

The resulting AUC is comparable to previous forensic studies that achieved AUCs on average in the range of 0.65$-$0.78 using non-algorithmic RAIs \cite{desmarais2016performance, douglas2003evaluation, singh2011comparative}.

\subsubsection{Prediction changes due to the RAI}

The observed probability of a participant changing a prediction after observing the machine prediction is %20,35\% (19.42\% in G1 and 21.33\% in G2).
20\% (19\% in G1 and 21\% in G2).
%
Crowdsourced participants revised their prediction in about 26\% of the cases they examined (27\% in G1, 25\% in G2).
%
Domain experts revised their prediction in 37\% of the cases, and data scientists in only 13\% of the cases.

Figure~\ref{fig:learning} shows the average difference in risk predictions by human and algorithm for each case. %As can be seen the risk predictions issued by participants are in general higher than the ones produced by the RAI, particularly at the beginning. 
%
Targeted participants started with predictions that were in general as high as those of the crowdsourced groups and equally far from those of the RAI.
%
As they progress through the evaluation tasks, participants tend to align more and more their predictions with the machine predictions (even in their initial predictions) and the difference between initial and revised predictions diminishes.
%
For the last three cases, the crowdsourced group's predictions, which are already close to the machine predictions, do not change, while the targeted group maintains a larger difference between initial and revised predictions.
%

By comparing the average AUC in Figure~\ref{fig:auc_group} and Table~\ref{tab:results1}, we can see that revised predictions from crowdsourced groups tend to be more accurate than their initial ones in terms of AUC.
%
This difference is significant for R1's G2 ($p<0.1$) and for R2's G1 ($p<0.05$), as shown in Table \ref{tab:ttests} (in Supplementary Material~\ref{ann:accuracy-per-subgroup}). For the targeted groups, we see an improvement in the range from +0.01 to +0.09 AUC points on average.
%
In almost all cases, revised predictions by the treatment groups are more accurate than those of the control groups. However, few of these differences are statistically significant. % (in Table~\ref{tab:ttests}).

In general, the average self-reported confidence is in the range 3.5-3.9 out of 5.0 (1.0=least confident, 5.0=most confident), and basically does not change from the initial to the final prediction.
%
The self-reported confidence of crowdworkers is, by a small but statistically significant margin ($p<0.001$), higher than the one of targeted participants (see Supplementary Material~\ref{ann:self-reported-confidence}).

\subsubsection{Preferred level of automation}

%\begin{figure}
%  \includegraphics[width=0.25\textwidth]{reliance_control.png}
%  \caption{Distribution of answers about level of automation. Only control group.}
%  \label{fig:reliance_control}
%\end{figure}
\begin{figure}[!tbp]
  \centering
  \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{change_accuracy.pdf}
  \caption{AUC of participant predictions before and after algorithmic support for participants who received algorithmic support (excludes control group).}
%  \mynote[from=Marzieh]{By accuracy, you mean AUC? This figure is only cited in the discussion. Shouldn't it be explained in the results firs?}
%  \inote{this should go to Appendix and referenced by \ref{fig:auc_group}.}
 % \mynote[from = Songül]{I think it can stay as it doesn't take away space.}
  \label{fig:accuracydist}
  \Description{Shows a scatterplot with individual accuracy, both for initial and final prediction (after algorithm suggestion).}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{change_reliance.pdf}
  \caption{Distribution of answers about level of automation for participants who received algorithmic support (excludes control group).} 
 % \mynote[from=Marzieh]{I would prefer to change the x and y axis labels to "accepted level of automation at the start of the study" and "accepted level of automation at the end of the study". Or add an explanation in the caption to show that "initial" and "final" mean "start" and "end" of the study.}
  \label{fig:reliance_nocontrol}
  \Description{Shows a scatterplot divided in sections regarding their answer for the level of automation survey. In the plot, the initial values and the final values are compared.}
  \end{minipage}
  \vspace{-3pt}
\end{figure}

As shown in Figure~\ref{fig:reliance_nocontrol}, most participants prefer an intermediate level of automation, between levels 2-4 on a scale of 5 levels. While data scientists had an initial level of acceptance with a broader range (levels 1-4), domain experts limited their answers to a more narrow set of choices in intermediate levels of acceptance (levels 2-3).
%
The same figure also shows that most of the treated groups reduce their preferred level of automation after the experiment, meaning they prefer more expert involvement and less reliance on machine predictions.

On average, however, the desired level of acceptance for targeted groups concentrated in the middle-low part of the scale: 32\% of the data scientists and 48\% of the domain experts selected level 3 (``the computational system suggests one option, but the expert can provide an alternative option'').
%
Level 2 (``the computational system suggests some options, but it is the expert who defines the risk level''), was the option selected by 36\% of the surveyed data scientists and 38\% of the domain experts. 
%
Details can be found in Supplementary Material~\ref{ann:preferred-level-of-automation}, and the description of the automation levels can be found in Supplementary Material~\ref{ann:automationlevel}.

\subsection{Independent variables}

\subsubsection{Self-reported importance of risk items}
\label{importanceofriskitems}
Having asked to select the top 3 items (risk factors) that participants considered in their risk prediction, we find that crowdsourced and targeted participants tend to select the same 10-11 (out of 23) items as more important than the rest.
%
However, among these top 10 items we find that domain experts prefer dynamic factors (i.e., factors that can change), such as %\textit{``pro-criminal/antisocial attitude''} and 
\textit{``limited response to psychological treatment''}, 
%
while data scientists and crowdsourced participants refer more often than domain experts to static factors (i.e., factors that cannot change), such as \textit{``history of violence''} %, ``violent base offense''} and \textit{``childhood adjustment disorders''} 
%
%\mynote[from=Marzieh]{According to Figure \ref{fig:items_important} and Table \ref{tab:top5_items}, I think all groups mostly consider dynamic items as important features.}
(details are in Figure \ref{fig:items_important} and Table \ref{tab:top5_items} in  Supplementary Material~\ref{ann:items-considered-most-important}).

\subsubsection{Numerical information (R1)}

According to Figure~\ref{fig:auc_group}, adding numerical values to the categorical scale does not change the AUC. In G1, where only categorical information is shown, the AUC of revised predictions is slightly higher than the revised predictions in G2, where categorical and numerical values are shown: 0.62 against 0.61 AUC.

\subsubsection{Risk scales (R2 and Targeted)} \label{subsubsec:scales}

The results of R2 show that for the initial prediction, the absolute scale (G1) leads to slightly lower AUC compared to the relative scale (G2) (0.58 against 0.61 AUC).
%
However, with algorithmic support, the absolute scale leads to higher AUC than the relative scale (0.67 against 0.62 AUC).
%
Neither of these differences is statistically significant.
%
Additionally, the average AUC of the R2 control group (0.65) is fairly high, and the only higher AUC observation is in the revised predictions using the absolute scale (0.67).
%
The revised and some initial predictions of the targeted participants using the absolute scale %, where risk is displayed as a probability of recidivism, 
significantly outperform all the R1 groups, as well as the R2 groups ($p<0.05$, see Table~\ref{tab:ttests} in Supplementary Material~\ref{ann:accuracy-per-subgroup}).

\subsubsection{Additional variables}

With respect to \emph{numeracy}, over 60\% of the crowdsourced participants answered correctly 2 or 3 out of the 3 test questions.
%
The targeted group had more respondents answering all 3 numeracy questions correctly than crowdworkers, as shown in Table~\ref{tab:demographics}: 96\% of data scientists obtained results in the highest scores (68\% in the top score), while only 59\% of domain experts obtained similar results (52\% in the top score).
%
We find no correlation between participants' numeracy and their accuracy. 
%
The correlation between \emph{decision making style} and \emph{emotional state} with accuracy is not significant either (results are in Supplementary Material~\ref{ann:gdms-vas}). 

==> Riscanvi paper - experiment with humans/07-qualitative-study.tex <==
\section{Qualitative study}
\label{sec:qualitative-study}

The last study is a qualitative study using focus groups, i.e., groups of participants having a focused discussion on a particular topic \cite{morgan1998focus}.
%
The focus groups help us interpret the quantitative results from the targeted study, by listening to and learning from participants' experiences and opinions.

\subsection{Participants and procedure}

Participants (9 women, 4 men) were recruited from the \emph{targeted} experiment, and due to their busy schedules, divided into four groups (FG1-FG4) as follows:
\textbf{FG1} (N=3) data scientists; \textbf{FG2} (N=4) domain experts, students from criminology in undergraduate and master levels; \textbf{FG3} (N=2) and \textbf{FG4} (N=4) domain experts working with the Department of Justice, most of them psychologists.

While we did not want to give too much structure to the conversation, to try to uncover new perspectives that we had not thought about, we did prepare a series of questions to stimulate a discussion (available in Supplementary Material \ref{ann:focusgroup}). 
%
The questions address participants' experience with algorithmic predictions and RAIs, their opinion about different scales and categorical/numerical presentation, their understanding of risk factors, and their desired level of automation.
%
Each session lasted between 60 and 90 minutes and was held online. Following the protocol approved by our Ethics Review Board, participants were asked for their consent to participate and to have the meeting recorded and transcribed. 
%
The language of the focus group was the local language spoken in \Catalonia;  % Spanish -- SPAIN
the quotes we present in the next section were taken from our transcriptions and paraphrased in English.

\subsection{Findings}

%The insights from the focus groups are vast and would require additional space to reproduce. 
We focus on our research questions, but note that there were many other insightful comments during the focus groups.

\subsubsection{Professional background}

All participants were aware that some demographics are over/under represented among prison populations, and thus expected that a RAI trained on such data may lead to discriminatory outcomes.
%
However, the way in which data science participants approached risk prediction was to a large extent based on considering a set of ``anchors'' or prototypes \cite[p. 13]{Scurich2012b}:
``I think about a maximum and a minimum risk. The minimum would be like a person who stole for the first time [...] %and who has a low level, [...] % that is how I see it and that is how I am analyzing everything, and 
%the medium would be someone with multiple robberies, or rape [...]
the maximum would be a killer'' (FG1.1).
%the medium since is in between, it would be like a constant robbery with rape, and the maximum would be a killer psychopath. % This is how I justify my predictions" 
% FG1.1 = FG1-PM
%
In general, data scientists did not question the presented case characteristics, but domain experts did.
%
Participants in FG3 and FG4 indicated that the risk items, which in \RisCanvi only have three levels (Yes/Maybe/No), do not accurately represent the reality of inmates
%
and they were missing the ability to explore or negotiate the risk items during the case evaluations.
% 
Furthermore, they indicated that, during the assignment of levels to risk factors, they sometimes ``compensate'' higher values in one item with lower values in other items, %when coding, nuances in one variable are sometimes ``compensated'' by professionals in other variables 
%
%For instance, if a case worker was hesitant to code a risk factor as ``Yes'', s/he would be more likely to code another risk factor as ``No'', 
such that the final risk score matches what they would consider appropriate for the evaluated person.
%
One participant (FG4.1) %FG4.1 = FG4-TF
said that personal biases may also affect the coding of items, as some professionals adopt a more punitive approach, while others take a more protective or rehabilitative approach.
%
Other domain experts agreed with this perspective.
%In general, domain experts were aware that the process of encoding data for the RAI was influenced by professional biases and subjectivity.
%
Therefore, most professionals expressed the need for teams reviews and validation mechanisms for risk factor codings. 
%They also indicated this was the main reason why items need to be agreed by team reviews and validated afterwards. 

Among domain experts, the psychologists we interviewed were the most concerned about the evidence they collect and the representation of the actual risk. 
%
To them, RAIs are tools that add objectivity to their case reports,
%They agreed that RAIs are tools that help bring objectivity to their arguments, but were concerned about how to present evidence 
but their focus was on \emph{how} to present evidence to judges, since these might discard professional reports in favor of the RAI's outcome. % bring objectivity = "crear objetividad"?
%
% Removed from Manuel, not really related to RQs
%A participant (FG4.2) % FG4.1 = FG4-GB
%indicated that sometimes judges do not pay attention to the text of \RisCanvi reports, and only used the \RisCanvi risk level for making decisions. 
%
%The discussions made it clear that professionals with experience on \RisCanvi ad other RAIs were aware of the processes by which data was encoded, and took advantage of the instrument as a mediator and as an element for negotiation and consensus.
%
Overall, for domain experts RAIs such as \RisCanvi should be used by a group of experienced evaluators checking one another, and not by one professional alone. 
%For domain experts \RisCanvi and other RAIs were never supposed to be used by one individual professional alone, but always as part of the work of a group of experienced evaluators that can question each other and the results. 

\subsubsection{Interpreting numbers}

All participants had some training in statistics, and stated that they understand numerical expressions well. %Social workers and psychologists are used to categorical levels since RisCanvi is expressed only in three categories (low, medium, and high), 
Generally, participants preferred a relative scale (e.g., 3.7/10.0) over an absolute scale (e.g., 37\%). %However, they acknowledge that criminology education involves training in statistics and probabilities.
 
 %One of the interesting discussions with the domain experts was about how they interpret a probability of recidivism in an individual case.
It is noteworthy how domain experts interpret probabilities.
 %
 First, %they assume that having an 
 extremely low risks were considered unlikely in practice, since almost everyone can commit a crime at some point.
 %
 Second, all interviewed domain experts stated that recidivism risk cannot be eliminated but it could be reduced to an acceptably low level (e.g., reducing the risk from 37\% to 20\%).
 %
 This emphasis on risk reduction is in line with the ``interventions over predictions'' debate in the literature~\cite{barabas2018interventions}.
 %Removed by Songül on 2021-11-08
 %Given the RAI encoded information, profesionals working with inmates can consider specific treatments related to the factors that can be changed by arresstees (e.g. lack of plans for the future, or drug dependency).  \mynote[from=Manuel]{We can sumarize paragraph above.}
%
Third, domain experts consider a recidivism risk of above 30\% as high, and a reason for concern. A risk above 50\% %was considered very high and 
was considered difficult -but not impossible- to reduce by treatment/interventions.
%
Overall, domain experts thought of different ranges on the risk spectrum along which inmates are placed.
%
Data scientists, too, considered different risk ranges, and for some of them even a 50\% recidivism risk was not considered ``high.''
%This is the opposite to what computer scientists stated, because for them a 50\% probability is not as high because they understand numbers in frequency terms. 

\subsubsection{Interaction with machine predictions and calibration}

Many participants admitted that they went quickly, and without giving it much thought, through the first few evaluations. %"one was answering automatically". 
%
However, they also noticed that they slowed down to rethink when they felt contested by the algorithm, i.e., when their risk assessment was far from the algorithm's prediction. %No matter if the algorithm was more precise or not, 
%Participants reacted to differences to the algorithm independent of its precision. 
Data scientists indicated that they reacted to such differences by simply adjusting the risk to half-way between their initial prediction and the one of the algorithm. %if there was a difference between their prediction and the suggested, they simply set their corrected score to the average of their initial score and the machine score. 
Domain experts indicated to react similarly in some cases, %. But they also said that they 
but they also stressed that they kept their initial prediction when they felt confident about it.

Some of the domain experts %we interviewed 
believed that they were interacting with exactly the same \RisCanvi algorithm they use, despite a clear indication in the introduction of the study that this was another algorithm.
%
We believe their experience with the real \RisCanvi %quite possibly 
affected their disposition to rely on the machine predictions we presented.

\subsubsection{Preferred level of automation}
 
Overall, domain experts and data scientists differed in the level of automation they would prefer, with data scientists being more open to automation.  %always wanted to have the last word in deciding, but computer scientists were more open. 
%
For instance, participant FG1.2 % FG1.2 = FG1-MV
believed that an algorithm could improve enough to make almost-autonomous decisions ``in the future.'' 
%
This participant considered the errors that could be made by the algorithm were ``acceptable.'' %said that, even if it gets wrong a few times, it is comparable to the errors made by humans, therefore it is acceptable.
%
In contrast, e.g., FG1.3 % FG1.3 = FG1-IK
was sceptical about using an algorithm for automated decision-making 
because of the impossibility to solve all algorithm-specific errors. % regarding false positives and false negatives. 


All participants agreed that algorithmic support is useful in many instances, e.g., to %Some argued that it helps to have a support for 
contrast their own predictions, to give them a chance to rethink them, or to provide reassurance about them.
%
Domain experts also considered them useful to train new case workers in writing evaluations.
%
In that regard, participants from FG1 and FG2, expressed that the ``objectivity''  of the algorithm could help reduce the effect of the ``emotional'' response to the evidence by the professional who is evaluating. 

%Removed by Manuel: this is just a speculation, maybe in discussion is better.
%If this is the case, algorithmic support may lead to increased confidence in their predictions. 
%Nevertheless, no participant reconsidered their acceptance level for using an automated system after the discussion.
%

Participants also acknowledged the risk of ``relying too much'' on the algorithm, leading to reduced professional responsibility: ``The decision you make is yours, it is yours with your biases and everything, which also brings experience because it sometimes helps you to be aware and review your own prejudices'' (FG2.1). %FG2.1 = FG2-UR 
%
 %%removed by Songül
%At the same time, they were worried that the machine reproduces societal biases and that the algorithm cannot change as society changes (e.g. in sensible topics as gender violence, abortion, drugs, etc). As a consequence, they expected that the algorithm should be continually updated. 
%alternative by Songül
%
Another drawback of using a RAI noted by participants was the concern that it may reproduce potentially outdated societal prejudices.
%
To address this concern, domain experts expected frequent updates to the algorithms.


==> Riscanvi paper - experiment with humans/08-discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\textbf{RQ1: Under which conditions do participants using a RAI to predict recidivism achieve the highest predictive accuracy?} 
%\textbf{RQ1: Under which conditions does a human decision maker achieve the best accuracy?} % and Brier score?}
%\mynote[from = Songül]{Brier score does not appear in the results sections. We should either include it in the results sections or remove any discussion or mentioning of it, e.g. in Section 3.1}

%\subsection{Accuracy}
Overall, our findings suggest that human decision makers achieve higher accuracy for their risk-assessment when they are supported by an algorithm.
%
%Despite lower accuracy levels before the treatment, 
Almost all treatment groups achieve a higher AUC than their corresponding control group after the treatment, although some of these differences are not statistically significant, particularly in the case of crowdsourced participants (Figures \ref{fig:auc_group} and \ref{fig:accuracydist}). %The algorithm affects human accuracy in general, as evidenced by the before-after changes in accuracy in Figures \ref{fig:auc_group} and \ref{fig:accuracydist}, and also 
%
The algorithm also influences human predictions for each decision and over time, as shown in Figure \ref{fig:learning}. This further suggests that algorithmic support establishes reference points to human predictions.
%
The lower accuracy of the initial predictions of treatment group participants compared to control group participants is noteworthy.
%
One possible explanation for this is that treated participants put less effort in their initial predictions in anticipation of algorithmic support and a potential opportunity to revise their initial prediction. 
%Removed by Songül
%Some studies show that human participants accommodate their answers to what algorithms suggested in previous cases. In the same direction, the platform used in our studies helps participants to adjust their accuracy as shown in Figure~\ref{fig:accuracydist}. 
%We can speculate that people accommodated their perception of risk to what the algorithm was suggesting, as further indicated by some participants in the focus group. Even more, after adjusting the dataset in the second round, which increased both the human and the system accuracy, we see a clear increase in the AUC for all groups.
%we can argue that there are cases more easy to identify both for humans and for the machine (see figure \ref{fig:casespredictions}).

%Removed by Songül
%In terms of performance, crowdsourced participants were outperformed by the algorithm which goes in line with \cite{Green2019a, Lin2020, Bansak2019, Dressel2018}. But, for the targeted group most of the groups outperformed the algorithm (see Figure \ref{fig:auc_group}), 
The finding that targeted participants (domain experts and data scientists) outperform crowdsourced participants contradicts the idea that crowdsourced participants are comparable to domain experts or professionals when testing RAIs. This highlights the importance of testing RAIs in the context of professional knowledge, training and usage. 

%We also acknowledge that the groups from the crowdsourced study, who are not experts in the subject,
%Removed by Songül
%However, computer scientists performed similar to domain experts. Looking for an explanation, a better understanding of statistics could be a reason for having a good performance. Nevertheless, the numeracy score did not differ between crowdsourced and targeted groups, an exhaustive study should be done to confirm that hypothesis.
%Finally, our experiments yield some evidence for the ideas that %limiting information \cite{Lin2020, Tan2018a} and %% Manuel: I'm not sure that we tested this because all experiments provided almost same information.
Finally, using an absolute rather than a relative scale leads to more accurate predictions. The focus group further confirmed the preference of professionals for the absolute scale as the one closer to the real application. % and triggered a discussion on the presentation of risk scores as categorical risk levels, which to professionals seemed to limit their abilities.
%
Our findings agree with Hilton et al. \cite{ZoeHilton2008}, who found that risk categories are generally hard to agree upon across professions and individuals,
%
and also with Hanson et al. \cite{Hanson2017}, who found that categories can be effective following a common agreement in correspondence to ranges of the absolute probability of recidivism.
%
Thus, further studies should focus on the underlying support of numerical information in helping ground categorical distinctions for predictive risk assessment. 
%
%Removed by Songül
%Regarding different forms of showing risk scores, and in coincidence with our findings, other studies found that less information could help to encourage a better performance in risk prediction \cite{Lin2020, Tan2018a}. In addition, the debate during the focus groups about the limits of risk levels re-enforce also the idea by \cite{ZoeHilton2008} that category boundaries are hard to agree on among experts, that is constrained by the way that they use \RisCanvi and their professional training and goal.

%Some see it as a tool oriented to make a psychological profile and focus more on the individual items, while others use it to obtain predictions about the future behaviour of the evaluated individuals and focus more on the final risk score \cite{Heilbrun1999}. %But we consider that using both, numerical expressions, the categorical levels and the scales, help them to improve their discussion regarding levels, and help them to accommodate towards a more precise prediction.

%Removed by Songül
%The differences between the results with the relative and absolute scales were minor. In general, the results with absolute scale were more accurate. We found statistical difference between targeted and crowdsourced groups when comparing the experimental groups using absolute scale \footnote{A paired t-test shows a p-value less than 0,0001. Detailed information is available in Table \ref{tab:ttests}}. Also, as participants declared, it is more representative to the actual professional activity to have an absolute scale. In addition, participants valued positively the use of a 5-level scales rather than 3-level which is currently used in \RisCanvi.  

%\textbf{RQ2: To what extent do participants rely in their decision-making on an automated system to predict recidivism? }
\noindent\textbf{RQ2: To what extent do participants rely on the RAI to predict recidivism?}
%\subsection{Accepted level of automation}


%Removed by Songül
%The results from the accepted level of automation shows that participants are sceptic about extremes, and in general, they choose a middle or low level of automation. Even more, all the experimental groups have a tendency to downgrade their acceptance of automation (see Figure~\ref{fig:reliance_nocontrol}). 
%We did not find any correlation between their accuracy and the acceptance of automation. 
%There are multiple explanations for this: First, participants could consider themselves capable enough of making decisions without any assistance, given that accuracy has not significantly changed. Second, if their experience was that the machine was providing results far from their prediction, it could be not trustworthy enough. 
%Third, even when accuracy increased in all levels it was mainly for those that started with low accuracy, meaning that most participants already had a good level of accuracy to begin with. 
In line with previous studies (e.g., \cite{Tan2018a}) humans and algorithms tend to agree on very low and very high risk cases (see Supplementary Material~\ref{ann:casesel}, particularly Figure \ref{fig:casespredictions}),
but there are cases that are difficult to predict for humans, for algorithms, or for both.
%
A promising next step would be to identify cases that are clearly difficult for the machine, and or are potentially difficult to humans. In these cases one could more safely defer to humans, or ask them to invest more time in a specific evaluation, improving efficiency in the design of human-algorithm decision processes. 

Our findings show that %rather than fully automating decisions by the RAI or completely banning any use of an RAI in this context,
participants prefer a partially automated assistance with a large degree of human discretion.
%
In addition, all experimental groups tend to downgrade the acceptable level of automation after the experiment (see Figure~\ref{fig:reliance_nocontrol}).
%
Explanations for this could be that the differences between human and machine predictions caused the participants to realize strong human oversight was more necessary than what they initially thought.
%
%The responses do not differ significantly between control and treatment groups (see Appendix \ref{ann:additionalresults}).


%Removed by Songül
%We discussed this topic with participants in the focus group and all participants agreed that they felt more confident about their decision with the algorithm's assistance in cases where their score disagreed with the algorithm's prediction. This could be an interesting point of departure when designing collaborative human-algorithm decision processes.
%Removed by Songül
%The focus group revealed that participants welcome the assistance of an algorithm, but they remain sceptical of providing total control to an automated system. We must say that the difference between levels 2 and 3 of automation acceptance are very small. However, participants prefer to get only one suggestion from the algorithm, because more open options would be confusing.

Finally, the focus group discussions revealed that professionals' reliance in an algorithm could be increased when the algorithm providers ensure good prediction performance and frequent system updates corresponding to new societal and institutional developments. This suggests that \RisCanvi and possibly other RAIs are elements of negotiation that should be taken with care and without assuming its outcome as objective, and that need frequent updates and audits.
% This confirms the need for frequent quality updates of algorithmic applications in high risk contexts such as criminal justice. 

%Removed by Songül
%From another point of view, it is evident that for any RAI and also any algorithm-supported system, methods and data should be periodically updated to encourage trust and reliance. In the case of the criminal system, laws change over time and so do societal norms and dynamics. Any data-driven system should incorporate this fact and update data and parameters regularly.

%The necessity of updating evidence collection, variables and concepts makes that RAIs get outdated. As a consequence, by training algorithms with historical data means that the algorithms could not represent current state of affairs, putting accuracy in danger by introducing historical biases. Thus, to ensure reliance and acceptance, algorithms should provide rigorous outputs. 

%\todo[from=ChaTo]{Next paragraph needs to be integrated}

%The reduction on the desired automation level can be associated with the interpretation of the definition of each of the levels (see Appendix \ref{ann:surveytemplate}) but also with the own experience during the study. The responses do not differ significantly between control and treatment group (see Appendix \ref{ann:additionalresults}).

%\todo[from=ChaTo]{Next paragraph needs to be integrated}

%The fact that groups with categorical and numerical information perform as well as groups that only receive categorical informaiton (R1) is in line with \cite{Lin2020} who show that humans perform relatively well with a limited amount of information.


==> Riscanvi paper - experiment with humans/09-limitations.tex <==
\vspace{-4mm}
\section{Limitations and Future Work}
\label{sec:limitations}

This paper has to be seen in light of some limitations. 
%
First, %as everyone in the Machine Learning would agree, it has become apparent that bad data cannot be used to assess a model .
the dataset used for training the algorithm has some drawbacks. %On the one side, the data has a high number of low-risk inmates, which might be representative of prison population but tends to bias the trained algorithm. 
It has only about 597 cases, 
%and 
%For one, the amount of data used for training the algorithm (approximately 900 cases) 
%cannot be representative of the entire prison population, which may affect accuracy. %Therefore, the accuracy of the algorithm is not as high as it could be.
which may affect the algorithm's accuracy; however, we note that its AUC-ROC is in line with that of most recidivism prediction tools.
%
We also note that in this dataset the ground-truth label is \textit{re-arrest} and not \textit{re-offense}, and  re-arrest is not necessarily a good proxy for re-offense and further exhibits racial and geographical disparities \cite{fogliato2021validity}.
%
Since the focus of this study is the assessment of user behaviour (not the algorithm), we do not expect these drawbacks to notably affect our main results.
%
Second, in line with previous work, this study focuses on accuracy as a measure of algorithmic performance. % following previous studies in the subject,
However, decision support algorithms can be evaluated in many different ways \cite{Sambasivan2021}. %and more research that compares alternative performance metrics in similar user studies could shed light on the extent of the consequences of this limitation.
%Nevertheless, such limitation was justified because it was our intention to study user behaviour, not the algorithm.  
%
Third, Figure \ref{fig:learning} shows that participants are still calibrating their predictions after the training phase as they progress through the evaluation tasks, suggesting that the initial training phase may have been to short. %While this is an indicator of how the interaction with RAIs affects human predictions, this can also suggest that the initial training phase may have been to short. %Designers of user studies usually face a trade-off between using time to familiarize participants with the experiment and ensuring high completion rates. 
The impact should be limited as the majority of the cases are evaluated after this learning curve has flattened.

The generalization of this work to other contexts is restricted by other factors. As usual in experimental user studies, %rather than other studies that equal laypeople to crowdworkers, we need to acknowledge that the
the crowdsourced participants are not representative of the overall population.
%
Table \ref{tab:demographics} shows that most have university-level education and good numeracy. 
%
Further, we only recruited participants in a single country. Thus, the pool of users might not exhibit a large cultural diversity, a factor that could bias outcomes~\cite{Beale2008, Lee2012}.
%
However, we also remark that crime and recidivism is different in different criminal systems and jurisdictions, and hence RAIs should be evaluated with careful attention to their context \cite{Selbst2019}. 
%
Sample size may be another limitation. While the size of our participant pool in the crowdsourced study (N=247, N=146) is in line with previous work, the number of participants in the targeted study (N=54) is relatively small.
%
%\todo{Power analysis https://towardsdatascience.com/introduction-to-power-analysis-in-python-e7b748dfa26}
Despite these limitations in sample size, our results suggest consistent and in some cases statistically significant differences in the outcomes between crowdsourced and targeted participants.

Future research is needed to explore the reasons and conditions of these differences. This is particularly important in the public sector, where there is a lack of evidence on how algorithms affect public policies \cite{Zuiderwijk2021}. %For example, in the recidivism prediction context, decision making processes are open, negotiated and mediated, and if a RAI is used for reducing inter-professional communication rather to increase it, it can have adverse effects in decision quality.
There is a clear need to pay attention to the usage contexts and the ways in which RAIs are deployed, to reduce the risks of automation and understand better in which conditions the assistance of an algorithm can be most helpful. 



==> Riscanvi paper - experiment with humans/paired_ttests.tex <==
\begin{table}[ht] 
\centering
\begin{tabular}{lcrr}
  \hline
 Group 1 & Relation & Group 2 & p-value \\ 
  \hline
Crowd R1- Control       & < & Targeted - G1 Before & 0.018 \\ 
Crowd R1- Control     & < & Targeted - G1 After & 0.002 \\ 
Crowd R1- Control     & < & Targeted - G2 After & 0.016 \\ 
Crowd R1 - G1 Before  & < & Targeted - G1 Before & 0.002 \\ 
Crowd R1 - G1 Before  & < & Targeted - G1 After & 0.002 \\ 
Crowd R1 - G1 Before  & < & Targeted - G2 After & 0.006 \\ 
Crowd R1 - G2 Before  & < & Targeted - G1 Before & 0.004 \\ 
Crowd R1 - G2 Before  & < & Crowd R1 - G1 After & 0.020 \\ 
Crowd R1 - G2 Before  & < & Crowd R1 - G2 After & 0.092 \\ 
%  10 & 0.58 & 0.75 & Crowd R1 - G2 Before & < & Targeted - G1 After & 0.002 \\ 
%  11 & 0.58 & 0.68 & Crowd R1 - G2 Before & < & Targeted - G2 After & 0.004 \\ 
Crowd R2- Control    & \textcolor{red}{>} & Crowd R2 - G1 Before & 0.082 \\ 
Crowd R2- Control    & < & Targeted - G1 After & 0.010 \\ 
Crowd R2 - G1 Before & < & Targeted - G1 Before & 0.004 \\ 
Crowd R2 - G1 Before & < & Crowd R2 - G1 After & 0.012 \\ 
Crowd R2 - G1 Before & < & Targeted - G1 After & 0.002 \\ 
Crowd R2 - G1 Before & < & Targeted - G2 After & 0.018 \\ 
Crowd R2 - G2 Before & < & Targeted - G1 Before & 0.042 \\ 
Crowd R2 - G2 Before & < & Crowd R2 - G1 After & 0.044 \\ 
Crowd R2 - G2 Before & < & Targeted - G1 After & 0.002 \\ 
Crowd R2 - G2 Before & < & Targeted - G2 After & 0.034 \\ 
%  22 & 0.67 & 0.62 & Targeted - G1 Before & \textcolor{red}{>} & Crowd R1 - G1 After & 0.038 \\ 
%  23 & 0.67 & 0.61 & Targeted - G1 Before & \textcolor{red}{>} & Crowd R1 - G2 After & 0.020 \\ 
Targeted - G1 Before & \textcolor{red}{>} & Crowd R2 - G2 After & 0.088 \\ 
Targeted - G1 Before & < & Targeted - G1 After & 0.026 \\ 
Targeted - G2 Before & < & Targeted - G1 After & 0.004 \\ 
%  27 & 0.62 & 0.75 & Crowd R1 - G1 After  & < & Targeted - G1 After & 0.002 \\ 
%  28 & 0.62 & 0.68 & Crowd R1 - G1 After  & < & Targeted - G2 After & 0.024 \\ 
%  29 & 0.61 & 0.75 & Crowd R1 - G2 After  & < & Targeted - G1 After & 0.002 \\ 
%  30 & 0.61 & 0.68 & Crowd R1 - G2 After  & < & Targeted - G2 After & 0.026 \\ 
Crowd R2 - G1 After  & < & Targeted - G1 After & 0.020 \\ 
Crowd R2 - G2 After  & < & Targeted - G1 After & 0.002 \\ 
Targeted - G1 After  & \textcolor{red}{>} & Targeted - G2 After & 0.058 \\ 
   \hline
   
\end{tabular}
\caption{Permutation t-tests for differences between AUC-ROC of subgroups, showing only differences that are significant at $p < 0.1$.
%
In most cases the relation is that crowdsourced groups are less accurate than targeted groups, and predictions before machine assistance are less accurate than predictions after machine assistance. Cases where this relationship is inverted are more rare. The relationship signs ($<,>$) indicate which group has a higher AUC.}\label{tab:ttests}
\end{table}


==> Riscanvi paper - experiment with humans/removed.tex <==
 

 \section{Removed from related work}
 
 These tools are differentiated by their degree of structure and human involvement in the final risk assessment which ranges from an unstructured ("clinical") assessment with high human involvement to a completely structured ("actuarial") assessment with lower human involvement. Fully actuarial instruments take over all four components of the violence risk assessment, from the (i) identification of empirically valid factors, to (ii) the determination of a method for scoring the individual risk factors, to (iii) developing a procedure to combine these scores, and finally to (iv) producing a numerical estimate of the risk \cite{skeem2011current}. Thus, when taking into account the human oversight aspect, the performance of RAIs depends on several aspects, such as the degree of structure, the design and presentation of the instrument and the involvement, and the experience and educational background of professionals working with the RAI. 

 %%%%% COMMMENT FROM MANUEL: I REMOVED THIS PARAGRAPH ABOVE, I THINK IT IS EXPLANATORY BUT NOT REALLY NEEDED IN THIS CONTEXT.
 
 \section{Removed from related work}
 
The participants in these studies, mainly recruited from crowdsourcing platforms, are asked to predict the probability of re-offense of different cases which are characterised by the features that are also used in the studied RAIs (e.g. criminal history factors). 

\section{Removed from the end of related work}

analyze the RAI comparing multiple populations and interpreting the results with experienced professionals. 
Our findings may lead to a deeper understanding about advantages and drawbacks of RAIs beyond their mere accuracy. 
We also discuss in depth the benefits and drawbacks of this type of RAI with people from different backgrounds, including experienced professionals. 

\subsection{Algorithm supported prediction of recidivism risk}


 
 Moreover, choosing the right performance metric to evaluate an algorithm is relevant to the extend that good performance in accuracy may not automatically imply or even counteracts good performance in terms of fairness \cite{miron2020evaluating}.  



\subsection{Risk communication}

An actuarial activity prescribe rules for scoring or coding information to generate numerical rankings with the goal to place individual offenders into specified risk categories. This opens the door to several topics that are presented as open discussions. 

The value of any risk assessment varies depending on the role and the experience of each professional working with the RAI.  It also has its limits regarding interpretation and context of use. Thus, the decision on which actuarial information is presented and how is shown is not trivial, but part of a longstanding discussion. Therefore, the design of the decision interface, i.e. the way risk assessments are communicated and integrated in the decision process, can play a crucial role in shaping effective human-algorithm interaction. 


In the professional practice, RAIs are used differently by different professionals \cite{Heilbrun1999}. On the one hand, RAIs are just prediction-oriented tools, where the outcome is taken solely to inform a decision objectively. For example, judges are more inclined to rely on individual information, rather than on statistical outputs, disregarding the actuarial assessment. 

On the other hand, professionals such social workers or psychologists, understand RAIs as management-oriented tools. The outcome is a baseline for defining a treatment for an inmate, or a tool for communicating with other professionals.


Because different instruments appear to yield different outcomes based on different risk factors, there is a current danger for algorithms created upon already existing datasets. Interfaces, devices and features are commonly used in specific contexts, defined accordingly to contemporary social values \cite{Suchman2007}. By interpreting an algorithm' outcome, it could have a complete different meaning \cite{Jung2013}. That is because values have meaning for actuarial clinicians with that tool in mind. It is true that overlapping factors such as criminal history or criminal attitudes can bring concordances. But, the weight and definition of each risk factor is defined by the practices in specific contexts. 
%

Algorithmic guidance doesn’t need to be 100\% precise, but should be contextualized. (Acharya, A., Howes, A., Baber, C., & Marshall, T.  2018)

\section{Description of accuracy}

As a metric, \emph{accuracy} is simply the probability of issuing a prediction that is supported by some ground truth, typically measured in a particular reference dataset. This is computed as the ratio between the number of correct predictions and the total number of predictions done.
%
In probabilistic, score-based predicting algorithms, measuring accuracy typically requires a threshold. This metric is also affected by the prevalence of different categories in the data; for instance if 99\% of the cases are positive, a system that merely predicts ``positive'' for all cases is 99\% accurate.

\section{AUC and Brier Score}

For example, a classification system with an AUC of 0.5 classifies a randomly drawn positive example, e.g. a high-risk recidivist, as a high-risk case in 50\% of the cases. Thus, an AUC of 0.5 is equivalent to random classification, while an AUC of 1.0 is equivalent to a correct classification at every instance.
% 
For instance, if the AUC of a RAI is 0.7, in 70\% of the pairs involving a recidivist and a non-recidivist, the risk score produced by the RAI for the recidivist is higher than the score of the non-recidivist.
%
%removed by Songül (All about brier score)
A disadvantage of the AUC metric is that it is not sensitive to the scale of the predictions; for instance, if we multiply all the risk scores by a constant, the AUC does not change \cite{Bansak2019}. This means that a predictor with large calibration error (i.e. when the predicted probability does not reflect the true probability) could still yield a high AUC.
%\mynote[from=Marzieh]{Why does the previous sentence mean this?}
%
To avoid this, we also use the \textbf{Brier score}, which is the mean squared error of the forecast. Hence, the lower the Brier score for a set of predictions, the better the predictions.
%
We use AUC in all of our experiments to provide an easier comparison with other relevant studies, and additionally the Brier Score to consider a potential calibration error.

\subsection{Accuracy}

%
% Removed by ChaTo on 2021-09-27
Using a metric to measure accuracy further allows for clear and simple comparisons of the decision performance of different groups and decision making systems. Therefore, accuracy is also a popular measure in the literature when human decision making is compared to algorithmic decision making. In this paper, we also use accuracy to compare the decision performance between groups with different backgrounds, i.e. laypeople vs. undergraduate students of relevant research fields and professionals who actually work with RAIs. 
%
However, it should be noted that neither is there one universal metric that represents \textit{accuracy}, nor is accuracy the only qualitatively relevant indicator for RAIs. 

%
%
As reviewed in the previous section, many studies compare human vs. algorithmic prediction. 
As \cite{Green2020} stated, we cannot expect that human decisions can be improved by helping them to having higher algorithmic-supported accuracy. Instead, we can understand what conditions are helping to improve their risk predictions. 
We are also interested in comparing the performance between specific groups, differentiating from laypeople to experts in domains such as data science and criminal psychology.
We acknowledge such limitations, but because AUC-ROC is useful for comparing to other studies, we decided to adopt both metrics for fulfilling our needs at this dimension.\\

\subsubsection{INFORMATION}
\textcolor{red}{In the risk communication literature, research about information overload and its relation with accuracy is scarce. Few studies mention the importance of complementary information for making high-stake decisions. In contrast, behavioural studies state that information overload can reduce human accuracy. In \cite{Balfe2018} it is shown that reducing user workload can have a higher impact than system precision. }\mynote[from=Manuel]{This part is not related with numerical factors, but we need to justify}
We decided to test different combinations of categorical levels and numerical expressions (see Figure \ref{fig:scales}) , which is described in the experimental setup for each study. \\

%Removed by Songül on 2021-11-08
Risk can be expressed in the form of scores, and also probability percentages. We speculated with presenting information in both approaches to find relations between numeracy abilities and professional background with the interpretation of such numerical expressions. 

\section{Removed from methods -- it was repetitive}
%
Using non-experts for studying domain-specific risk assessment tools for recidivism is an open debate, even when statistical methods can improve the performance of non-experts \cite{Bansak2019}. 
%
However, crowdsourced experiments are common in behoavioural experiments with RAIs \cite{Green2020,VanBerkel2019,Yin2019,Dressel2018,Lin2020}, and it is necessary for us to consider non-experts not only to compare our results with other studies but also to compare our findings between experts and non-experts. 

\section{Old table}

\begin{tabular}{l|cl|cl|cl}
         Type $\rightarrow$ 
         & \multicolumn{2}{c|}{\textbf{Crowdsourced}}
         & \multicolumn{2}{c|}{\textbf{Crowdsourced}}
         & \multicolumn{2}{c}{\textbf{Targeted}} \\
         Group $\downarrow$ 
         & {N} & {Round 1}
         & {N} & {Round 2} 
         & {N} &  ~ \\
         \hline
         Control & 48 & \texttt{[C:ABS]} & 17 & \texttt{[C:ABS]} & - & - \\
         G1 & 100 & \texttt{[C:ABS:CAT]} &  66 & \texttt{[C:ABS:CAT+NUM]} & 36 &  \texttt{[T:ABS:CAT+NUM]} \\
         G2 & 99 & \texttt{[C:ABS:CAT+NUM]} &  63 & \texttt{[C:REL:CAT+NUM]} & 18 & \texttt{[T:REL:CAT+NUM]} \\
         \hline
         Total
             & 247 &
             & 146 & 
             & 54 \\
         \multicolumn{7}{l}{\footnotesize * We named groups in \texttt{[]} using the following encoding: \texttt{C} or \texttt{T} for indicating if belongs to Crowdsourced or Targeted study. }\\
         \multicolumn{7}{l}{{\footnotesize  \texttt{A} for absolute scale and \texttt{R} for relative scale. \texttt{LVL} if it includes risk levels. \texttt{SCR} if includes 0 to 10 risk scores, or \texttt{\%} if includes}}\\
         \multicolumn{7}{l}{{\footnotesize the probability of risk expressed in percentage. }}\\
         
    \end{tabular}

    
\section{Removed from crowdsourcing results}

% Next paragraph removed by ChaTo -- these groups cannot be compared

As mentioned in the paragraph above, in round 2 the control group has a higher AUC than the treatment group with the relative scale (0.65 vs. 0.62). This shows, too, how some additional information can sometimes even be misleading to human decision makers. 

In the second round (R2), we perceive a general improvement in all the predictions (Figure \ref{fig:auc_group}), probably due to the new dataset of cases for which the algorithm also had a higher AUC (see  \ref{subsubsec:cases}). While the control group had a better accuracy for the initial prediction, it was outperformed by the experimental groups after receiving algorithmic support in the second screen (see Figure \ref{fig:auc_group}).


\mynote[from=MAnuel]{From annex}
\section{Additional Studies}
\subsection{Preliminary studies}
\label{ann:preliminary}

% see https://docs.google.com/presentation/d/18YjtNyIlev9x3Tf3V0CJIVPH38Ab-ZVpVb7gkwsSuKQ/edit#slide=id.ga5ed635af8_0_0
Before running our studies, we developed a preliminary where we tested the platform and other different variables, and defining different experimental groups. In one of them presented only categorical risk (low, middle, high) and in other, we experimented with explainable methods.  However, we haven't seen any significant difference between the three experimental groups. But, we perceived an emergent trend towards a better accuracy with the algorithmic guidance. We used this step to assess as many cases as possible to allow us to select and filter the cases for the first study (process detailed in Appendix \ref{ann:casesel}).

In the beginning of the project we run preliminary studies with different testers to evaluate its aesthetics and its interpretation of the platform as well as the cases to be included. We run our survey with 30 participants from which only 27 successfully finished the experiment, plus another 4 that participated in the control group (31 in total). Also, we filter participants by their country of residence to select only those who live in Spain. This was a deliberated decision because criminal systems can differ from one country to another. 

\subsection{Explainability treatment}
During the crowdsourced study we experimented with a ML explainer to increase the amount of information. We used AnchorsLIME \cite{Ribeiro2018} over a group of additional 94 participants (G3) to test if a more advanced explanation can help to improve accuracy. But we haven't found any considerable differences. A more deep work should be done to test different explainers, specially because just one explanation obscures and can affect the notions of justice \cite{Binns2018}.

\subsubsection{Experimental Setup}
For this preliminary study, we differentiated 4 groups:
\begin{itemize}
    \item Control Group: Does not shows any prediction
    \item Experimental Group 1: shows only the predicted risk level (low, mid or high)
    \item Experimental Group 2: shows the predicted risk score + risk level
    %\item Experimental Group 3: shows the predicted risk score + risk level + explanation with 3 main features (generated using a AnchorsLIME explainer \cite{Ribeiro2018})
\end{itemize}

\subsubsection{Results}
From the explainability treatment, we received 94 participations and we obtained a AUC-ROC of 0.580 without algorithmic support and 0.609 after receiving the algorithmic prediction. In comparison with the other experimental groups (before: 0.598 and 0.576; after: 0.621 and 0.607, respectively) we consider that there is no statistical difference in treatment. 

\section{Qualitative -- Domain experts}

On the contrary, the domain experts we interviewed were more conscious about some socio-technical limitations of using RAIs. For example, taking as evidence the data that appeared in their screens. Moreover, some participants reported that, because RisCanvi asks for encoding the items (e.g. only accepting Yes, No, Maybe), professionals that collect the evidence as their daily work can decide to adapt their report to "compensate" one variable over another in order to obtain an output that corresponds to their professional opinion. This reveals what could be a tendency among experts, to provide inputs to the system to keep it in line with their background knowledge. 
Another participant (FG4-TF), with more than 30 years of experience, stated that he thinks that professionals can choose to be punishers or protectors for the inmates, and collect the results accordingly in order to influence the final result. That is to say, that some biases are embedded when evidence is collected and the process of encoding data for the RAI is, sometimes, altered to fit professionals' opinion. Nevertheless, usually evidence and reports are agreed by team reviews and validators afterwards. 

Psychologists from the domain expert groups were more concerned about the evidence they have collected and the representation of the actual risk. They expressed more concern about how to present evidence to judges, and they agree that RAIs are tools that help to create objectivity around their arguments. A participant (FG4-GB) highlights that sometimes judges do not pay attention to their report and only take the RisCanvi score for making decisions. 

The discussions make clear that the professionals who had experience with RAIs, are aware of all the processes for which data is encoded and decoded and may take advantage of the instrument itself as a mediator. Similarly, participants from FG3 and FG4 stated that some items have limited options that do not represent the reality of the inmates, and they cannot interrogate nor negotiate such variables.
These findings suggest that RisCanvi in particular, but also other RAIs, are elements of negotiation that should be taken with care and do not assume its outcome as objective, that also need constant update and audit. Such instruments are never used only by one individual professional but always by a group of experienced evaluators that can question the results. 

\section*{Removed from conclusions}

Through this user study on the use of algorithmic support in recidivism risk assessment, 
%
we observed that algorithmic support leads to small but consistent gains in predictive accuracy.
%
These improvements are to a large extent due to participants changing some of their predictions to be more aligned with those of the algorithm.
%
Statistically significant differences were observed between crowdsourced and targeted participants (domain experts and data scientists).
%

In general, participants in our experiments considered that algorithmic support was useful, and domain experts stressed various benefits  of algorithmic support beyond accuracy: as a tool to communicate and negotiate risk assessment between different professionals, as a training tool, as a means to establish a common language, and as a mechanism to trigger self-reflection in decision making, double-checking difficult cases.
%
At the same time, most participants rejected the idea of fully-automated recidivism risk prediction, and became more skeptical about automation after completing the experiment.
%



==> Riscanvi paper - experiment with humans/tab_confidence.tex <==
 \begin{tabular}{ll|cc}
    \toprule
      Study & Group & Before & After \\
    \midrule
    Crowd (R2) & G1 & 3.89 $\pm$ 0.89 & 3.82  $\pm$ 0.98 \\
    Crowd (R2) & G2 & 3.90  $\pm$ 0.77 & 3.82  $\pm$ 0.95 \\
    Targeted & G1 & 3.48  $\pm$ 0.71 & 3.45  $\pm$ 0.85 \\
    Targeted & G2 & 3.57  $\pm$ 0.81 & 3.52  $\pm$ 0.97 \\
    \midrule
    Targeted & Domain Experts & 3.47 $\pm$ 0.73 & 3.52  $\pm$ 0.82 \\
    Targeted & Data Scientists & 3.55 $\pm$ 0.76 & 3.43  $\pm$ 1.04 \\
    \bottomrule
  \end{tabular}


==> Riscanvi paper - experiment with humans/tab_confidence_ttest.tex <==

\begin{tabular}{lll}
\toprule Group 1 & Group 2 & p-value \\\midrule
Crowd R2 - G1 Initial & Targeted - G1 Initial & $<$0.001**** \\ 
Crowd R2 - G2 Initial & Targeted - G2 Initial & $<$0.001**** \\ 
Crowd R2 - G2 Initial & Targeted - G1 Initial & $<$0.001**** \\ 
Crowd R2 - G2 Initial & Targeted - G2 Initial & $<$0.001**** \\ 
Crowd R2 - G2 Initial & Targeted - G2 Final & $<$0.001****\\ 
Crowd R2 - G1 Initial & Targeted - G1 Final	& $<$0.001****\\ 
Crowd R2 - G1 Initial & Targeted - G2 Final	& $<$0.001****\\ 
Crowd R2 - G2 Initial & Targeted - G1 Final	& $<$0.001****\\
\toprule
\end{tabular}


==> Riscanvi paper - experiment with humans/tab_demographics.tex <==
 \begin{tabular}{ll|cccc}
    \toprule
      & & \textbf{Crowd. (R1)} & \textbf{Crowd. (R2)} & \textbf{Dom.Exp} & \textbf{Data.Sci} \\
      & & N=247 & N=146 & N=29 & N=25\\
    \midrule
    \textbf{Gender} & Male &  61.0\%  & 54.3\% & 20.7\% & 40.0\% \\
       & Female &  48.4\% & 45.7\% & 79.3\% & 56.0\%   \\
       & Other &  0.6\%  & 0.0\% & 0.0\% & 4.0\% \\
    \midrule
       \textbf{Education}  
       %& Elementary & 0.9\% & 0.8\%  & 0.0\% \\
        & Secondary & 19.3\% & 15.5\% & 3.5\% & 20.0\% \\
        & Undergraduate & 57.5\% & 68.2\%  & 48.2\% & 56.0\% \\
        & Postgraduate & 22.3\% & 15.5\% & 48.3\% & 24.0\% \\
    \midrule
        \textbf{Age} & 18-25 & 44.3\% & 53.5\%  & 55.2\%  &  76.0\% \\
        & 26-33 & 25.2\% & 24.8\% & 10.3\% & 20.0\% \\
        & 34-45 & 19.6\% & 12.4\% & 13.8\% & 4.0\% \\
        & 45-75 & 10.9\% &  9.2\% & 20.7\% & 0.0\% \\
 
    \midrule
    % I'm using numeracy as the number of correct answers in the numeracy test -- ChaTo
       \textbf{Numeracy}  & 0 (lowest) & 11.2\% & 18.5\% & 17.2\% &  4.0\% \\
    & 1 & 15.0\% & 20.5\% & 24.1\% & 0.0\% \\
    & 2 & 24.0\% & 22.0\% & 6.9\% & 28.0\% \\
    & 3 (highest) & 49.8\% & 39.0\% & 51.7\% & 68.0\% \\
    \bottomrule
  \end{tabular}


==> Riscanvi paper - experiment with humans/tab_experimentalgroups.tex <==
\begin{table}[h]
\small
    \begin{tabular}{l|cl|cl|cl}
         Type $\rightarrow$ 
         & \multicolumn{2}{c|}{\textbf{Crowdsourced}}
         & \multicolumn{2}{c|}{\textbf{Crowdsourced}}
         & \multicolumn{2}{c}{\textbf{Targeted}} \\
         Group $\downarrow$ 
         & {N} & {Round 1}
         & {N} & {Round 2} 
         & {N} &  ~ \\
         \hline
         Control 
         & 48 & Abs. scale
         & 17 & Abs. scale 
         & - & - 
         \\
         G1 
         & 100 & Abs. scale / categorical
         &  66 & Abs. scale / cat. and num. 
         & 36 &  Abs. scale / cat. and num.
         \\
         G2 
         & 99 & Abs. scale / cat. and num.
         &  63 & Rel. scale / cat. and num.
         & 18 & Rel. scale / cat. and num.
         \\
         \hline 
         Total
             & 247 &
             & 146 & 
             & 54 \\
    \end{tabular}
    \caption{Characteristics of the experimental groups.
    %
    The control groups received no machine predictions.
    %
    The treatment groups received machine predictions.
    %
    G1 used an absolute scale indicating a probability (0\% to 100\%); 
    G2 used a relative scale indicating a score (0 to 10).}
    \label{tab:experimentalgroups}
\end{table}


==> removed.tex <==
 

 \section{Removed from related work}
 
 These tools are differentiated by their degree of structure and human involvement in the final risk assessment which ranges from an unstructured ("clinical") assessment with high human involvement to a completely structured ("actuarial") assessment with lower human involvement. Fully actuarial instruments take over all four components of the violence risk assessment, from the (i) identification of empirically valid factors, to (ii) the determination of a method for scoring the individual risk factors, to (iii) developing a procedure to combine these scores, and finally to (iv) producing a numerical estimate of the risk \cite{skeem2011current}. Thus, when taking into account the human oversight aspect, the performance of RAIs depends on several aspects, such as the degree of structure, the design and presentation of the instrument and the involvement, and the experience and educational background of professionals working with the RAI. 

 %%%%% COMMMENT FROM MANUEL: I REMOVED THIS PARAGRAPH ABOVE, I THINK IT IS EXPLANATORY BUT NOT REALLY NEEDED IN THIS CONTEXT.
 
 \section{Removed from related work}
 
The participants in these studies, mainly recruited from crowdsourcing platforms, are asked to predict the probability of re-offense of different cases which are characterised by the features that are also used in the studied RAIs (e.g. criminal history factors). 

\section{Removed from the end of related work}

analyze the RAI comparing multiple populations and interpreting the results with experienced professionals. 
Our findings may lead to a deeper understanding about advantages and drawbacks of RAIs beyond their mere accuracy. 
We also discuss in depth the benefits and drawbacks of this type of RAI with people from different backgrounds, including experienced professionals. 

\subsection{Algorithm supported prediction of recidivism risk}


 
 Moreover, choosing the right performance metric to evaluate an algorithm is relevant to the extend that good performance in accuracy may not automatically imply or even counteracts good performance in terms of fairness \cite{miron2020evaluating}.  



\subsection{Risk communication}

An actuarial activity prescribe rules for scoring or coding information to generate numerical rankings with the goal to place individual offenders into specified risk categories. This opens the door to several topics that are presented as open discussions. 

The value of any risk assessment varies depending on the role and the experience of each professional working with the RAI.  It also has its limits regarding interpretation and context of use. Thus, the decision on which actuarial information is presented and how is shown is not trivial, but part of a longstanding discussion. Therefore, the design of the decision interface, i.e. the way risk assessments are communicated and integrated in the decision process, can play a crucial role in shaping effective human-algorithm interaction. 


In the professional practice, RAIs are used differently by different professionals \cite{Heilbrun1999}. On the one hand, RAIs are just prediction-oriented tools, where the outcome is taken solely to inform a decision objectively. For example, judges are more inclined to rely on individual information, rather than on statistical outputs, disregarding the actuarial assessment. 

On the other hand, professionals such social workers or psychologists, understand RAIs as management-oriented tools. The outcome is a baseline for defining a treatment for an inmate, or a tool for communicating with other professionals.


Because different instruments appear to yield different outcomes based on different risk factors, there is a current danger for algorithms created upon already existing datasets. Interfaces, devices and features are commonly used in specific contexts, defined accordingly to contemporary social values \cite{Suchman2007}. By interpreting an algorithm' outcome, it could have a complete different meaning \cite{Jung2013}. That is because values have meaning for actuarial clinicians with that tool in mind. It is true that overlapping factors such as criminal history or criminal attitudes can bring concordances. But, the weight and definition of each risk factor is defined by the practices in specific contexts. 
%

Algorithmic guidance doesn’t need to be 100\% precise, but should be contextualized. (Acharya, A., Howes, A., Baber, C., & Marshall, T.  2018)

\section{Description of accuracy}

As a metric, \emph{accuracy} is simply the probability of issuing a prediction that is supported by some ground truth, typically measured in a particular reference dataset. This is computed as the ratio between the number of correct predictions and the total number of predictions done.
%
In probabilistic, score-based predicting algorithms, measuring accuracy typically requires a threshold. This metric is also affected by the prevalence of different categories in the data; for instance if 99\% of the cases are positive, a system that merely predicts ``positive'' for all cases is 99\% accurate.

\section{AUC and Brier Score}

For example, a classification system with an AUC of 0.5 classifies a randomly drawn positive example, e.g. a high-risk recidivist, as a high-risk case in 50\% of the cases. Thus, an AUC of 0.5 is equivalent to random classification, while an AUC of 1.0 is equivalent to a correct classification at every instance.
% 
For instance, if the AUC of a RAI is 0.7, in 70\% of the pairs involving a recidivist and a non-recidivist, the risk score produced by the RAI for the recidivist is higher than the score of the non-recidivist.
%
%removed by Songül (All about brier score)
A disadvantage of the AUC metric is that it is not sensitive to the scale of the predictions; for instance, if we multiply all the risk scores by a constant, the AUC does not change \cite{Bansak2019}. This means that a predictor with large calibration error (i.e. when the predicted probability does not reflect the true probability) could still yield a high AUC.
%\mynote[from=Marzieh]{Why does the previous sentence mean this?}
%
To avoid this, we also use the \textbf{Brier score}, which is the mean squared error of the forecast. Hence, the lower the Brier score for a set of predictions, the better the predictions.
%
We use AUC in all of our experiments to provide an easier comparison with other relevant studies, and additionally the Brier Score to consider a potential calibration error.

\subsection{Accuracy}

%
% Removed by ChaTo on 2021-09-27
Using a metric to measure accuracy further allows for clear and simple comparisons of the decision performance of different groups and decision making systems. Therefore, accuracy is also a popular measure in the literature when human decision making is compared to algorithmic decision making. In this paper, we also use accuracy to compare the decision performance between groups with different backgrounds, i.e. laypeople vs. undergraduate students of relevant research fields and professionals who actually work with RAIs. 
%
However, it should be noted that neither is there one universal metric that represents \textit{accuracy}, nor is accuracy the only qualitatively relevant indicator for RAIs. 

%
%
As reviewed in the previous section, many studies compare human vs. algorithmic prediction. 
As \cite{Green2020} stated, we cannot expect that human decisions can be improved by helping them to having higher algorithmic-supported accuracy. Instead, we can understand what conditions are helping to improve their risk predictions. 
We are also interested in comparing the performance between specific groups, differentiating from laypeople to experts in domains such as data science and criminal psychology.
We acknowledge such limitations, but because AUC-ROC is useful for comparing to other studies, we decided to adopt both metrics for fulfilling our needs at this dimension.\\

\subsubsection{INFORMATION}
\textcolor{red}{In the risk communication literature, research about information overload and its relation with accuracy is scarce. Few studies mention the importance of complementary information for making high-stake decisions. In contrast, behavioural studies state that information overload can reduce human accuracy. In \cite{Balfe2018} it is shown that reducing user workload can have a higher impact than system precision. }\mynote[from=Manuel]{This part is not related with numerical factors, but we need to justify}
We decided to test different combinations of categorical levels and numerical expressions (see Figure \ref{fig:scales}) , which is described in the experimental setup for each study. \\

%Removed by Songül on 2021-11-08
Risk can be expressed in the form of scores, and also probability percentages. We speculated with presenting information in both approaches to find relations between numeracy abilities and professional background with the interpretation of such numerical expressions. 

\section{Removed from methods -- it was repetitive}
%
Using non-experts for studying domain-specific risk assessment tools for recidivism is an open debate, even when statistical methods can improve the performance of non-experts \cite{Bansak2019}. 
%
However, crowdsourced experiments are common in behoavioural experiments with RAIs \cite{Green2020,VanBerkel2019,Yin2019,Dressel2018,Lin2020}, and it is necessary for us to consider non-experts not only to compare our results with other studies but also to compare our findings between experts and non-experts. 

\section{Old table}

\begin{tabular}{l|cl|cl|cl}
         Type $\rightarrow$ 
         & \multicolumn{2}{c|}{\textbf{Crowdsourced}}
         & \multicolumn{2}{c|}{\textbf{Crowdsourced}}
         & \multicolumn{2}{c}{\textbf{Targeted}} \\
         Group $\downarrow$ 
         & {N} & {Round 1}
         & {N} & {Round 2} 
         & {N} &  ~ \\
         \hline
         Control & 48 & \texttt{[C:ABS]} & 17 & \texttt{[C:ABS]} & - & - \\
         G1 & 100 & \texttt{[C:ABS:CAT]} &  66 & \texttt{[C:ABS:CAT+NUM]} & 36 &  \texttt{[T:ABS:CAT+NUM]} \\
         G2 & 99 & \texttt{[C:ABS:CAT+NUM]} &  63 & \texttt{[C:REL:CAT+NUM]} & 18 & \texttt{[T:REL:CAT+NUM]} \\
         \hline
         Total
             & 247 &
             & 146 & 
             & 54 \\
         \multicolumn{7}{l}{\footnotesize * We named groups in \texttt{[]} using the following encoding: \texttt{C} or \texttt{T} for indicating if belongs to Crowdsourced or Targeted study. }\\
         \multicolumn{7}{l}{{\footnotesize  \texttt{A} for absolute scale and \texttt{R} for relative scale. \texttt{LVL} if it includes risk levels. \texttt{SCR} if includes 0 to 10 risk scores, or \texttt{\%} if includes}}\\
         \multicolumn{7}{l}{{\footnotesize the probability of risk expressed in percentage. }}\\
         
    \end{tabular}

    
\section{Removed from crowdsourcing results}

% Next paragraph removed by ChaTo -- these groups cannot be compared

As mentioned in the paragraph above, in round 2 the control group has a higher AUC than the treatment group with the relative scale (0.65 vs. 0.62). This shows, too, how some additional information can sometimes even be misleading to human decision makers. 

In the second round (R2), we perceive a general improvement in all the predictions (Figure \ref{fig:auc_group}), probably due to the new dataset of cases for which the algorithm also had a higher AUC (see  \ref{subsubsec:cases}). While the control group had a better accuracy for the initial prediction, it was outperformed by the experimental groups after receiving algorithmic support in the second screen (see Figure \ref{fig:auc_group}).


\mynote[from=MAnuel]{From annex}
\section{Additional Studies}
\subsection{Preliminary studies}
\label{ann:preliminary}

% see https://docs.google.com/presentation/d/18YjtNyIlev9x3Tf3V0CJIVPH38Ab-ZVpVb7gkwsSuKQ/edit#slide=id.ga5ed635af8_0_0
Before running our studies, we developed a preliminary where we tested the platform and other different variables, and defining different experimental groups. In one of them presented only categorical risk (low, middle, high) and in other, we experimented with explainable methods.  However, we haven't seen any significant difference between the three experimental groups. But, we perceived an emergent trend towards a better accuracy with the algorithmic guidance. We used this step to assess as many cases as possible to allow us to select and filter the cases for the first study (process detailed in Appendix \ref{ann:casesel}).

In the beginning of the project we run preliminary studies with different testers to evaluate its aesthetics and its interpretation of the platform as well as the cases to be included. We run our survey with 30 participants from which only 27 successfully finished the experiment, plus another 4 that participated in the control group (31 in total). Also, we filter participants by their country of residence to select only those who live in Spain. This was a deliberated decision because criminal systems can differ from one country to another. 

\subsection{Explainability treatment}
During the crowdsourced study we experimented with a ML explainer to increase the amount of information. We used AnchorsLIME \cite{Ribeiro2018} over a group of additional 94 participants (G3) to test if a more advanced explanation can help to improve accuracy. But we haven't found any considerable differences. A more deep work should be done to test different explainers, specially because just one explanation obscures and can affect the notions of justice \cite{Binns2018}.

\subsubsection{Experimental Setup}
For this preliminary study, we differentiated 4 groups:
\begin{itemize}
    \item Control Group: Does not shows any prediction
    \item Experimental Group 1: shows only the predicted risk level (low, mid or high)
    \item Experimental Group 2: shows the predicted risk score + risk level
    %\item Experimental Group 3: shows the predicted risk score + risk level + explanation with 3 main features (generated using a AnchorsLIME explainer \cite{Ribeiro2018})
\end{itemize}

\subsubsection{Results}
From the explainability treatment, we received 94 participations and we obtained a AUC-ROC of 0.580 without algorithmic support and 0.609 after receiving the algorithmic prediction. In comparison with the other experimental groups (before: 0.598 and 0.576; after: 0.621 and 0.607, respectively) we consider that there is no statistical difference in treatment. 

\section{Qualitative -- Domain experts}

On the contrary, the domain experts we interviewed were more conscious about some socio-technical limitations of using RAIs. For example, taking as evidence the data that appeared in their screens. Moreover, some participants reported that, because RisCanvi asks for encoding the items (e.g. only accepting Yes, No, Maybe), professionals that collect the evidence as their daily work can decide to adapt their report to "compensate" one variable over another in order to obtain an output that corresponds to their professional opinion. This reveals what could be a tendency among experts, to provide inputs to the system to keep it in line with their background knowledge. 
Another participant (FG4-TF), with more than 30 years of experience, stated that he thinks that professionals can choose to be punishers or protectors for the inmates, and collect the results accordingly in order to influence the final result. That is to say, that some biases are embedded when evidence is collected and the process of encoding data for the RAI is, sometimes, altered to fit professionals' opinion. Nevertheless, usually evidence and reports are agreed by team reviews and validators afterwards. 

Psychologists from the domain expert groups were more concerned about the evidence they have collected and the representation of the actual risk. They expressed more concern about how to present evidence to judges, and they agree that RAIs are tools that help to create objectivity around their arguments. A participant (FG4-GB) highlights that sometimes judges do not pay attention to their report and only take the RisCanvi score for making decisions. 

The discussions make clear that the professionals who had experience with RAIs, are aware of all the processes for which data is encoded and decoded and may take advantage of the instrument itself as a mediator. Similarly, participants from FG3 and FG4 stated that some items have limited options that do not represent the reality of the inmates, and they cannot interrogate nor negotiate such variables.
These findings suggest that RisCanvi in particular, but also other RAIs, are elements of negotiation that should be taken with care and do not assume its outcome as objective, that also need constant update and audit. Such instruments are never used only by one individual professional but always by a group of experienced evaluators that can question the results. 

\section*{Removed from conclusions}

Through this user study on the use of algorithmic support in recidivism risk assessment, 
%
we observed that algorithmic support leads to small but consistent gains in predictive accuracy.
%
These improvements are to a large extent due to participants changing some of their predictions to be more aligned with those of the algorithm.
%
Statistically significant differences were observed between crowdsourced and targeted participants (domain experts and data scientists).
%

In general, participants in our experiments considered that algorithmic support was useful, and domain experts stressed various benefits  of algorithmic support beyond accuracy: as a tool to communicate and negotiate risk assessment between different professionals, as a training tool, as a means to establish a common language, and as a mechanism to trigger self-reflection in decision making, double-checking difficult cases.
%
At the same time, most participants rejected the idea of fully-automated recidivism risk prediction, and became more skeptical about automation after completing the experiment.
%


